Cooperative Team Strategies for Multi-player Perimeter-Defense Games

This paper studies a variant of the multi-player reach-avoid game played between intruders and defenders with applications to perimeter defense. The intruder team tries to score by sending as many intruders as possible to the target area, while the defender team tries to minimize this score by intercepting them. Finding the optimal strategies of the game is challenging due to the high dimensionality of the joint state space, and the existing works have proposed approximation methods to reduce the design of the defense strategy into assignment problems. However they suffer from either suboptimal defender performance or computational complexity. Based on a novel decomposition method, this paper proposes a scalable (polynomial-time) assignment algorithm that accommodates cooperative behaviors and outperforms the existing defense strategies. For a certain class of initial configurations, we derive the exact score by showing that the lower bound provided by the intruder team matches the upper bound provided by the defender team, which also proves the optimality of the team strategies.

==> defense_algorithm.tex <==
\section{The LGR Defense Policy \label{sec:defense_policy}}
\noindent 
% This section proposes the defender team strategy that outperforms the existing MM and MIS policies.
% We present the LGR-defense algorithm and prove its performance guarantees.
% We then propose a defense strategy that captures all intruders when $\Qest=0$, with some additional conditions.
% Finally, we show that the score is bounded from above by $\Qest$ under a certain condition, indicating that 
% With these two results, we show that $\Qest$ is the exact outcome (equilibrium solution) of the game.


\subsection{Zero Score Game}
\noindent
We first show that any game with $\Qest>0$ can be reduced to a virtual game with $\Qest=0$ (\emph{zero score game}) by removing intruders selected by the following algorithm:
% Algorithm~\ref{alg:removal} presented below.
% ALGORITHM:
\begin{algorithm}[h]
\caption{Removal of uncapturable intruders \label{alg:removal}}
\begin{small}
\begin{algorithmic}[1]
\State Initialize: $\aignore=\emptyset$, and $i=1$ 
\While {$\Qest>0$}
    \State $Q_{new}\gets$ compute $\Qest$ without $\{A_i,\aignore \}$
    \If {$Q_{new} < \Qest$}
        \State Append $A_i$ to $\aignore$
        \State $\Qest\gets Q_{new}$
    \EndIf
    \State $i\gets i+1$
\EndWhile
\State {\bf Return}: $\aignore$
\end{algorithmic}
\end{small}
\end{algorithm}

The idea behind this removal is to ignore the intruders that cannot be captured, and make sure all other intruders will be captured.
The following lemma shows that exactly $\Qest$ intruders need to be removed to generate a zero score game.
\begin{lemma}\label{lem:removal}
Suppose $\Qest=n>0$, then there exists a set of $n$ intruders whose removal will generate a new game with $\Qest=0$.
\end{lemma}
\begin{proof}
When $\Qest>0$, one can show by contradiction that there exists at least one intruder whose removal reduces $\Qest$ by $1$.
(See \ref{} for more details.)
% The contradiction is derived by supposing that there is no such intruder, and showing that it leads to the existence of $\djset$ with $\Qint(\djset)>\Qest$, which contradicts with the optimality of $\Qest$ in \eqref{eq:Qest}.
% Suppose there is no intruder whose removal reduces $\Qest$.
% Then we can show that there exists a selection of disjoint sets $G'$ such that $Q(G')>Q(G^*)=\Qest$ (details omitted for page constraints), which contradicts with the optimality of $\Qest$ and $G^*$.
% We have shown
% We show by contradiction that there exists an intruder whose removal decreases $\Qest$ by one.
% Suppose there is no such intruder.
% Then there exists at least two sets $\djset_1^*$ and $\djset_2^*$ that gives the optimal score $Q(\djset_1^*) = Q(\djset_2^*) = \Qest$, with the constraint $\subteam_A^k\cap\subteam_A^l=\emptyset$ for $k\in\djset_1^*$ and $l\in\djset_2^*$, i.e., no common intruders.
% The two sets do not share any intruder because if they did, then the removal of the common intruder will reduce both $Q(\djset_1^*)$ and $Q(\djset_2^*)$.
% Now, take $k\in\djset_1^*$ with $q_k>0$ and consider merging it to $\djset_2^*$.
% If $\awinrc^k\cap\awinrc^l=\emptyset$ for $\forall\, l\in\djset_2^*$, then $\djset_3 = \{k,\djset_2^*\}$ is a valid disjoint set and it has $Q(\djset_3)>Q(\djset_2^*)$, which contradicts with the optimality of $\djset_2^*$.
% If $k$ intersects with $l\in\djset_2^*$, then let $m$ be the smallest LGR that contains both $k$ and $l$.
% Since the regions intersect, we have $n_D^m<n_D^k+n_D^l$.
% However, since they share no intruders, we have $n_A^m\geq n_A^k+n_A^l$.
% Therefore, $q_m= n_A^m-n_D^m > n_A^k+n_A^l- n_D^k-n_D^l = q_k+q_l$, which again contradicts with the optimality of $\djset_2^*$.
% The case when $k$ intersects with multiple LGRs in $\djset_2^*$ can be treated similarly.
After removing this intruder, the same argument still holds if $\Qest$ is still positive.
Repeating this process, the score $\Qest$ reduces to zero after removing $n$ intruders.
% Also, observe that the order of the removal does not affect the result.
% Consider the optimally selected disjoint set $\mf G^*$.
% For an LGR with $q_k\geq 1$ in $\mf G^*$, we show by contradiction that there exists an intruder whose removal makes $q_i\leq q_k-1$ for all $i$ such that $\awinrc^i\subseteq\awinrc^k$; i.e., $\Qest$ is reduced by one.
% Suppose there is no such intruder.  
% Then we should have at least two LGRs $\awinrc^i$ and $\awinrc^j$ contained in $\awinrc^k$ that satisfy the following conditions: (i) $q_i=q_j=q_k$, and  (ii) $\subteam_A^i\cap\subteam_A^j=\emptyset$.
% If the two LGRs are disjoint, then $q_i+q_j = 2q_k > q_k$ contradicts with the assumption that $k\in G^*$ (we would have $i,j\in \mf G^*$ instead).  
% If the two LGRs intersect, let $\awinrc^m\subseteq \awinrc^k$ be the smallest LGR that contains both $\awinrc^i$ and $\awinrc^j$.
% One can show that this leads to a contradiction $q_m>q_k$.
% After removing one intruder, we can choose the next LGR in $\mf G^*$ with $q>0$ and repeat the process until $q_k\leq0,\,\forall\,k$.  Since each removed intruder contributes to the reduction in $\Qest$, at most $\Qest$ intruders need to be removed.
\end{proof}

% Let $\aignore$ be a set of intruders with cardinality $|\aignore|=\Qest$, such that the removal of those intruders generate a new game with $\Qest=0$.
 Following the proof of Lemma~\ref{lem:removal}, we can find the set $\aignore$ in Algorithm~\ref{alg:removal} by visiting every intruder and asking whether it reduces $\Qest$ or not (Algorithm~\ref{alg:removal}).
Importantly, the answer remains the same whether $\Qest$ is already reduced or not.
Therefore, each intruder needs to be visited only once; Algorithm~\ref{alg:removal} terminates within less than $N_A$ iterations.
Since the bottleneck in the while loop is the computation of $\Qest$ (line 3), the time complexity is $O(N_AN_D^4)$.
% Every time the answer is yes, we remove that intruder from the game, and continue until $\Qest=0$.
% Assuming that the set $\djset^*$ is already known, the complexity is linear in $N_A$ since each intruder is visited only once.



\subsection{The LGR-defense Algorithm}
\noindent
The LGR defense strategy is presented in Algorithm~\ref{alg:LGRdefense}.
% ALGORITHM
\begin{algorithm}[h]
\caption{LGR Defense \label{alg:LGRdefense}}
\begin{small}
\begin{algorithmic}[1]
\State Remove uncapturable intruders using Algorithm~\ref{alg:removal}
\State Assign 2v1 defense using Algorithm~\ref{alg:2v1assignment}
\State Assign 1v1 defense using Algorithm~\ref{alg:1v1assignment}
\State {\bf Return}: assignments (i.e., direction of motion)
\end{algorithmic}
\end{small}
\end{algorithm}
% 
It is continuously run throughout the game to update the defender-intruder assignments that uniquely define each defender's direction of motion.
\edit{As illustrated in Sec.~\ref{sec:extended_engagements}, the assignments will dynamically change as the game evolves in time.}
% \todo{additional comment about dynamic aspect here}

First, Algorithm~\ref{alg:removal} removes/ignores intruders to generate a zero score game with $\Qest=0$. 
% the intruders that are guaranteed to score are ignored so that the defenders can focus on the rest. % (to be discussed in Sec.~\ref{sec:saddle_point}).
Then the cooperative 2v1 defense and the individual 1v1 defense are considered sequentially.
% To simplify the proofs in the sequel, 
In this paper, we restrict ourselves to the case when $\lgsi_k\leq 1,\,\forall\,k$ after the removal of uncapturable intruders.
The assignment of cooperative 2v1 games is presented in Algorithm~\ref{alg:2v1assignment}.
% ALGORITHM:
 \begin{algorithm}[h]
 \caption{Assign 2v1 Defense \label{alg:2v1assignment}}
 \begin{small}
 \begin{algorithmic}[1]
\State Initialize: $\mf A_\text{assgn}=\emptyset$, $\mf D_\text{2v1}=\emptyset$, and $\mf D_\text{1v1}=\dteam$
 \While{$\exists\,k$ s.t. $\lgsi_k \geq 1$}
\State $m \gets \argmax_k n_D^k$ for $k$ s.t. $\lgsi_k \geq 1$
     \State $A_j \gets$ select one intruder in $\dwinrp^m$
    %  \State Assign $A_j$ to the pair ($D_R^m,D_L^m$)
     \State Append $A_j$ to $\mf A_\text{assgn}$, and $m$ to $\mf D_\text{2v1}$
     \State Remove $D_R^m$ and $D_L^m$ from $\mf D_\text{1v1}$
     \State Recompute $\lgsi_k$ for all $k$ with $\ateam \setminus \mf A_\text{assgn}$
 \EndWhile
\State {\bf Return}: $\mf D_\text{2v1}$, $\mf D_\text{1v1}$ and $\mf A_\text{assgn}$
 \end{algorithmic}
 \end{small}
 \end{algorithm}
%

The I-LGRs with $\lgsi=1$ are visited sequentially from the largest to the smallest in terms of the subteam size.
In each iteration, one intruder in $\dwinrp$ is assigned to the boundary defenders (line 5) regardless of whether the defenders already have other 2v1 assignments or not, which potentially generates the \sequential\ structure.
The indices saved in $\dteam_\text{2v1}$ is sufficient to know which defender should perform a pincer movement with which pair.
The already assigned intruders are removed from the computation of $\lgsi$ (line 8), and the while loop terminates when all the I-LGRs have $\lgsi\leq 0$, which occurs in less than $N_A$ iterations.
Since the bottleneck in the while loop is the recalculation of $\lgsi$'s which is $O(N_D^2N_A)$, the time complexity of Algorithm~\ref{alg:2v1assignment} is $O(N_D^2N_A^2)$.

% ALGORITHM 1v1:
 \begin{algorithm}[h]
 \caption{Assign 1v1 Defense \label{alg:1v1assignment}}
 \begin{small}
 \begin{algorithmic}[1]
\State Inputs: $\ateam_\text{assgn}$, $\dteam_\text{2v1}$, and $\dteam_\text{1v1}$ 
 \State $\ateam_\text{1v1}\gets \ateam \setminus \ateam_\text{assgn}$
\State Initialize a bipartite graph with $\{\dteam_\text{1v1},\dteam_\text{2v1}\}$ and $\ateam_\text{1v1}$
 \For{$k$ in $\dteam_\text{2v1}$}
     \If {Inequality in Eq.~\eqref{eq:ineligible} is satisfied}
    %  	\State Draw edges to intruders in the \implicit\ zone
     	\State Draw edges to $\forall\,A_j$ s.t. $\mf x_{A_j}\in\dwinr(D_R^k)\cap\dwinr(D_L^k)$
     \EndIf
 \EndFor
 \For{$D_i$ in $\dteam_\text{1v1}$}
    %  \State Draw edges to intruders in the defender winning region
     \State Draw edges to $\forall\,A_j$ s.t. $\mf x_{A_j}\in\dwinr(D_i)$
 \EndFor
 \State Solve maximum matching and save the edges for $\dteam_\text{1v1}$
 \State {\bf Return}: 1v1 assignments (edges for $\dteam_\text{1v1}$)
 \end{algorithmic}
 \end{small}
 \end{algorithm}
%
When assigning 1v1 games, Algorithm~\ref{alg:1v1assignment} accounts for the \implicit\ structure.
The implicit assignment is still applicable to the pairs in \sequential\ structure, but with a restriction.
Noting that each structure involves $n+1$ defenders and $n$ intruders, we can only consider one additional ``implicit'' assignment, otherwise there will be more intruders than the defenders.
To guarantee capture, it is necessary and sufficient for the additional intruder to be in the \implicit\ zone of the outermost defender pair (e.g., $(D_k,D_j)$ in Fig.~\ref{fig:sequential_2v1}).
% We consider this by disqualifying a 2v1 defender pair, $\dboundary^k$, from having an \implicit\ if it satisfies the following condition:
% \bnl
% \begin{array}{l}
% (a)\; \exists\,m \text{\;with\;}\lgsi_m=1,\;\text{s.t.,}\;  \dboundary^k\cap\dboundary^m\neq\emptyset \text{\; and} \\
% (b)\; n_D^m > n_D^k.
% \end{array}
% \label{eq:ineligible}
% \enl
In summary, a 2v1 defender pair, $\dboundary^k$, can have an \implicit\ if $D_R^k$ or $D_L^k$ are not used in any other 2v1 defense that is associated to a larger I-LGR, i.e.,
% \begin{itemize}
%     \item[(a)] It does not share a defender with other 2v1 defenses; and
%     \item[(b)] It shares a defender with other 2v1 defenses, but 
% \end{itemize}
% \bnl
% \begin{array}{l}
% \text{$D_R^k$ or $D_L^k$ are not used in any other 2v1 defense}\\
% \text{that is associated to a larger I-LGR,}
% (a)\; \text{There is no overlapping assignment;} \text{\; or} \\
% (b)\; \text{Overlap with $\dboundary^m$,} \text{\;but\;} n_D^m < n_D^k.
% \end{array}
% \label{eq:ineligible}
% \enl
\bnl
n_D^k > n_D^m, \forall m\in \dteam_\text{2v1}\;\text{s.t.}, \dboundary^m\cap\dboundary^k\neq\emptyset
\label{eq:ineligible}
\enl

% Any intruder pair that does not satisfy this condition is eligible to have an implicit assignment.
The solution of the matching problem (line 9) only affects the behavior of the defenders in the set $\dteam_\text{1v1}$, but not the pairs in $\dteam_\text{2v1}$ because the assignments are only ``implicit'' for them.
This is why we only need the edges for $\dteam_\text{1v1}$.
The computational bottleneck in Algorithm~\ref{alg:1v1assignment} is the maximum matching, which is known to have efficient polynomial time algorithms \cite{Chen2017}.
Noting that $|\{\dteam_\text{1v1},\dteam_\text{2v1}\}|\leq N_D$ and $|\ateam_\text{1v1}|\leq N_A$, the number of nodes in the bipartite graph is at most $N_D+N_A$, which leads to $O((N_A+N_D)^w)$ time with $w<2.5$ \cite{Mucha2004}.
% The number of unique defenders involved in the 2v1 assignments, $N_D'$, is bounded by $|\dteam_\text{2v1}|\leq N_D'\leq 2|\dteam_\text{2v1}|$.



% % Figure: 
% \begin{figure}[t]
% \centering
% \includegraphics[width=.4\textwidth]
% {figures/assignment_example}
% \caption{
% }
% \label{fig:assignment_ex}
% \end{figure}
% %
% \todo{Use the figure in Simulation section to reduce space.}
Figure~\ref{fig:sim_example}a shows an example of the assignments given by Algorithm~\ref{alg:LGRdefense}.
Notice that a defender can have multiple 2v1 games assigned to it.
Algorithm~\ref{alg:2v1assignment} generated the \sequential\ structure involving $D_1,D_2,D_3$ and $D_4$.
% This is one of the main differences from the existing defense strategies (MM or MIS approach), and will be explained in detail in the next subsection.
%We will show that such overlapping assignments all require the same direction of motion from the defender, and will eventually dissolve into multiple 1v1 games.
% We will show that such overlapping assignments will eventually dissolve into multiple 1v1 games.
After the 2v1 assignments, $A_4$ and $A_5$ are left for 1v1 assignments.
The pair $(D_1,D_4)$ is eligible for the \implicit, and only $A_5$ is in the \implicit\ zone.
% Notice that intruder $A_5$ has no assignment at this time.
Therefore, the maximum matching in Algorithm~\ref{alg:1v1assignment} selects $A_4$ to be pursued by $D_5$ and leaves $A_5$ to be implicitly assigned to $(D_1,D_4)$.
% Another major difference from the existing defense policies is that, with our algorithm, even those intruders without explicit assignment at the current time can be shown to be captured when certain conditions are met.
% In fact, we will show in the next section that all intruders will be captured if $\Qest=0$ and $\lgsi_k\leq 1,\; \forall\, k$.
We will prove the performance guarantees in the remaining sections.



% Perfect defense
\subsection{Performance Guarantees} \label{sec:perfect_defense}
\noindent
This section proves that the LGR defense in Algorithm~\ref{alg:LGRdefense} achieves perfect defense (i.e., guarantees zero score $Q=0$) if $\Qest=0$ and $\lgsi_k\leq 1$.
% This section finds the configuration for which the LGR defense (Algorithm~\ref{alg:LGRdefense}) achieves perfect defense: i.e., guarantees zero score $Q=0$.


\begin{lemma}\label{lem:completeness}
If $\Qest=0$ and $\lgsi_k\leq 1$, then no intruder is unmarked: i.e.,
each intruder has either (i) 1v1 assignment, (ii) 2v1 assignment, or (iii) implicit assignment.
% In other words, each intruder has one of the following: (i) one defender dedicated to perform 1v1 defense, (ii) a pair of defenders performing 2v1 defense with possible assignment to other 2v1 games, or (iii) a unique pair of defenders with implicit assignment structure.
\end{lemma}
\begin{proof}
It suffices to show that, after Algorithm~\ref{alg:2v1assignment}, the intruders without 2v1 assignment gets either 1v1 or implicit assignment.
We use Hall's marriage theorem \cite{Hall} to show that the maximum matching in Algorithm~\ref{alg:1v1assignment} covers all the intruders.
% Let $X$ denote the set of intruders without 2v1 assignment.
For any subset $W\subseteq \ateam_\text{1v1}$, let $\mc{N}(W)$ denote the neighbor set: i.e., the subset of defenders that can capture at least one in $W$.
Hall's theorem states that all intruders in $\ateam_\text{1v1}$ are covered if $|W|\leq |\mc{N}(W)|$ for all $W\subseteq \ateam_\text{1v1}$.

For $|W|=1$, it is easy to see by contradiction that every intruder has at least one edge:
if an intruder has no edge, then the smallest I-LGR that contains it will have $\lgsi \geq 1$,
% if an intruder has no edge, it implies that 
% there exists an I-LGR with $\lgsi=1$, 
which contradicts with the termination of Algorithm~\ref{alg:2v1assignment}.
% Similarly for $|W|=2$, suppose there exists a pair of intruders with only one defender node that has edges to them.
% It is easy to see that this configuration also leads to the existence of an I-LGR with $\lgsi=1$.

%We have proved $|W|\leq |\mc{N}(W)|$ is true for $|W|=1$ and 2.
%Now, to use mathematical induction, we suppose the above inequality is true for $|W|=1,..,n$ and prove that it guarantees the condition for $|W|=n+1$.
Now, suppose the inequality is true for $|W|=1,..,n$.
We will prove that the inequality is also true for $|W|=n+1$:
If the bipartite graph can be separated into $m$ connected components involving intruder subsets $w_1,.. w_m$, then we have $|\mc{N}(W)|=\sum_i^m |\mc{N}(w_i)|$ because the defender nodes for each subset $w_i$ are disjoint.
Since we have $|\mc{N}(w_i)|\geq |w_i|$ from the supposition that the inequality is true for $|w_i|\leq n$, we obtain $|\mc{N}(W)| \geq \sum_i^m |w_i| = |W|$.
If the bipartite graph is connected and $|\mc{N}(W)|\leq n$, there exists an I-LGR whose defender subteam is $\mc{N}(W)$ and the intruder subteam is $W$.
% Now suppose $|\mc{N}(W)|=n$.
Then this region has the score $\lgsi\geq(n+1)-n=1$.
Since this contradicts with the termination of Algorithm~\ref{alg:2v1assignment}, we obtain $|\mc{N}(W)|\geq n+1=|W|$.
% For the case where the bipartite graph is connected, suppose that $|\mc{N}(W)|=n$.
% There exists an I-LGR whose defender subteam is $\mc{N}(W)$ and the intruder subteam is $W$.
% This region has the score $\lgsi=(n+1)-n=1$, which again contradicts with the completeness of the 2v1 assignment.

With mathematical induction, we have shown that $|W|\leq |\mc{N}(W)|$ for $W\subseteq \ateam_\text{1v1}$ with any size.
Therefore, maximum matching in Algorithm~\ref{alg:1v1assignment} covers all the intruders.
\end{proof}


\begin{lemma}\label{lem:sequential_2v1noconflict}
If $\Qest=0$ and $\lgsi_k\leq1,\,\forall\,k$, then the \sequential\ structure generated by Algorithm~\ref{alg:2v1assignment} has no conflict (see Definition~\ref{def:conflict}).
% : all overlapping 2v1 assignments require the same direction of motion from each intruder.
%Suppose Algorithm~\ref{alg:2v1assignment} assigned multiple 2v1 games to $\di$.
%If $\Qest=0$ and $\lgsi_k\leq1,\,\forall\,k$, then all those assignments require the same direction of motion by $\di$.
\end{lemma}
\begin{proof}
%If $D_i$ serves as the left (or right) boundary defender for all of the 2v1 assignments, then the required motion is the same for all.
%We show by contradiction that $D_i$ does not serve as the left and right boundary defender simultaneously.
%
For $\di$ to have conflicting 2v1 assignments, the following condition is necessary: $\di$ has two I-LGRs, $l$ and $r$ with $\lgsi_l=\lgsi_r=1$, where $D_R^l = \di$ and $D_L^r=\di$.
If $D_i$ gets both assignments, then there is a conflict.
% : $l$ and $r$ denote the indices of the LGRs that $\di$ serves as the left and right boundary defender, with $q_l=q_r=0$ and $\lgsi_l=\lgsi_r=1$.

Consider $\awinri^m\triangleq\awinri(D_R^r,D_L^l)$, which contains both $\awinri^l$ and $\awinri^r$.
The score satisfies $\lgsi_m\geq (n_D^l+1)+(n_D^r+1)-(n_D^l+n_D^r+1)=1$.
% From the condition of the lemma, we know $\lgsi_m=1$.
We also know $\Qest=0 \Rightarrow q_m=0$, implying that $\dwinrp^m$ has at least one intruder to be assigned to $\dboundary^m$.
Since this assignment reduces one intruder from either $l$ or $r$, $\di$ only needs to perform 2v1 defense for one of the two: i.e., $\di$ does not get both assignments.
\end{proof}

\begin{lemma}\label{lem:sequential_2v1resolve}
If $\Qest=0$ and $\lgsi_k\leq1,\,\forall\,k$, then all \sequential\ structure given by Algorithm~\ref{alg:2v1assignment} turn into 1v1 games \edit{before any intruder reaches the perimeter}.
\end{lemma}
\begin{proof}
There are no conflicting 2v1 assignments, by Lemma~\ref{lem:sequential_2v1noconflict}.
Looking at each 2v1 game separately, the defender pair performs optimally against the intruder.
Recalling the 2v1 analysis, the intruder in $\dwinrp$ will eventually move into the defender winning region of either of the two boundary defenders (Prop.~\ref{prop:pincer}).
Every time such transition occurs, the number of interrelated 2v1 game decreases, and we have additional 1v1 and/or implicit assignment configuration.

Importantly, observe that the transition occurs by the intruder leaving an I-LGR and not by entering a new I-LGR, which implies that the local game scores $q$ and $\lgsi$ are both non-increasing.
Therefore, the condition $\Qest=0$ and $\lgsi_k\leq1$ will be preserved after the transition.
Since the conditions for no conflict (Lemma~\ref{lem:sequential_2v1noconflict}) are still true, the next transition that reduces the number of 2v1 games occurs in finite time.
Repeating this process, we see that the \sequential\ structure will separate into multiple 1v1 games and non-overlapping 2v1 games possibly having a implicit assignment structure.
With the result from Lemma~\ref{lem:unassigned_defense1}, the proof is completed.
\end{proof}


\begin{theorem}\label{thm:perfect_defence}
If the initial configuration is such that $\Qest=0$ and $\lgsi_k\leq 1, \forall\,k$, then the LGR-defense (Algorithm~\ref{alg:LGRdefense}) guarantees perfect defense.
\end{theorem}
\begin{proof}
By construction, the unique 1v1 and 2v1 assignments guarantee capture.
The \implicit\ and \sequential\ also guarantee capture by Lemmas \ref{lem:unassigned_defense1}~and~\ref{lem:sequential_2v1resolve}.
Since all intruders have either one of the above assignments (Lemma~\ref{lem:completeness}), the capture of all intruders is guaranteed.
%The in intruders is gutrude of allers have either (i) a unique 1v1 assignment, (ii) 2v1 assignment, or (iii) no assignment.
%By construction, every 1v1 assignment guarantees capture.
%Lemmas~\ref{lem:unassigned_defense1} and \ref{lem:unassigned_defense2} prove that intruders with no assignment will all be captured. 
%Lemma~\ref{lem:sequential_2v1} and the discussion that follows prove that all 2v1 assignments will lead to capture.
\end{proof}



% Saddle point equilibrium
% \subsection{Saddle-point equilibrium}
% \label{sec:saddle_point}
% \noindent We summarize the results of this section.
We summarize the results of this section in the following:

\begin{theorem}
If $\hat{q}_k\leq 1\,\forall\,k$ after removing $\Qest$ intruders found by Algorithm~\ref{alg:removal}, then the LGR-defense policy $\mf u_D^*$ guarantees
\bql
Q(\mf z_0; \controlset_D^*,\controlset_A)\leq  \Qest(\mf z_0), \; \forall \, \controlset_A\in U_A,
\label{eq:uDguarantee}
\eql
where $U_A$ is the set of all permissible intruder strategies.
\end{theorem}
\begin{proof}
% The result immediately follows from Lemma~\ref{lem:removal} and Theorem~\ref{thm:perfect_defence}.
\todo{}
\end{proof}

Finally, the combination of the strategy $\mf u_A^*$ from Theorem~\ref{thm:Qlow} and $\mf u_D^*$ from Theorem~\ref{thm:perfect_defence} gives us the following result:
\begin{corollary}
If $\hat{q}_k\leq 1\,\forall\,k$ after removing $\Qest$ intruders found by Algorithm~\ref{alg:removal}, then
\bql
Q(\controlset_D^*,\controlset_A)\leq  Q(\controlset_D^*,\controlset_A^*) \leq Q(\controlset_D,\controlset_A^*),
\eql
i.e., the strategies $(\controlset_D^*,\controlset_A^*)$ are at a saddle-point equilibrium, and the value of the game is $Q^*(\mf z_0) = \Qest(\mf z_0)$.
\end{corollary}
If the intruders stick to $\controlset_A^*$, then the defender team cannot reduce the score by changing their strategy.
Similarly, if the defenders keep $\controlset_D^*$, then the intruders cannot increase the score by changing their strategy.
% This result indicates the optimality of the proposed strategy in the sense that any deviation does not improve the score as long as the opponent sticks to the equilibrium strategy.


==> defense_algorithm_originalstructure.tex <==
\section{The LGR Defense Policy \label{sec:defense_policy}}
\noindent This section proposes the defender team strategy (LGR-defense strategy) that outperforms the existing MM and MIS policies.
%We first present the algorithm and then prove the condition when all intruders are captured.
We present the LGR-defense algorithm and prove its performance guarantees.
Finally, we show that the score is bounded from above by $\Qest$ under a certain condition, indicating that $\Qest$ is the exact outcome (equilibrium solution) of the game.


\subsection{The LGR-defense Algorithm}
\noindent
The LGR defense strategy is presented in Algorithm~\ref{alg:LGRdefense}.
% ALGORITHM
\begin{algorithm}[t]
\caption{LGR Defense \label{alg:LGRdefense}}
\begin{small}
\begin{algorithmic}[1]
\State Remove uncapturable intruders using Algorithm~\ref{alg:removal}
\State Assign 2v1 defense using Algorithm~\ref{alg:2v1assignment}
\State Assign 1v1 defense using Algorithm~\ref{alg:1v1assignment}
\State {\bf Return}: assignments (i.e., direction of motion)
\end{algorithmic}
\end{small}
\end{algorithm}
% 
It is continuously run throughout the game to update the defender-intruder assignments that uniquely define each defender's direction of motion.
In the first line, the intruders that are guaranteed to score are ignored so that the defenders can focus on the rest (to be discussed in Sec.~\ref{sec:saddle_point}).
The cooperative 2v1 defense and the individual 1v1 defense are considered sequentially.
In this paper, we restrict ourselves to the case when $\lgsi_k\leq 1,\,\forall\,k$ after the removal of uncapturable intruders.

% ALGORITHM:
 \begin{algorithm}[h]
 \caption{Assign 2v1 Defense \label{alg:2v1assignment}}
 \begin{small}
 \begin{algorithmic}[1]
\State Initialize: $\mf A_\text{assgn}=\emptyset$, $\mf D_\text{2v1}=\emptyset$, and $\mf D_\text{1v1}=\dteam$
 \While{$\exists\,k$ s.t. $\lgsi_k \geq 1$}
\State $m \gets \argmax_k n_D^k$ for $k$ s.t. $\lgsi_k \geq 1$
     \State $A_j \gets$ select one intruder in $\dwinrp^m$
    %  \State Assign $A_j$ to the pair ($D_R^m,D_L^m$)
     \State Append $A_j$ to $\mf A_\text{assgn}$, and $m$ to $\mf D_\text{2v1}$
     \State Remove $D_R^m$ and $D_L^m$ from $\mf D_\text{1v1}$
     \State Recompute $\lgsi_k$ for all $k$ with $\ateam \setminus \mf A_\text{assgn}$
 \EndWhile
\State {\bf Return}: $\mf D_\text{2v1}$, $\mf D_\text{1v1}$ and $\mf A_\text{assgn}$
 \end{algorithmic}
 \end{small}
 \end{algorithm}
%
The assignment of cooperative 2v1 games is presented in Algorithm~\ref{alg:2v1assignment}.
The I-LGRs with $\lgsi=1$ are visited sequentially from the largest to the smallest in terms of the subteam size.
In each iteration, one intruder in $\dwinrp$ is assigned to the boundary defenders (line 5) regardless of whether the defenders already have other 2v1 assignments or not, which potentially generates the \sequential\ structure.
The indices saved in $\dteam_\text{2v1}$ is sufficient to know which defender should perform a pincer movement with which pair.
The already assigned intruders are removed from the computation of $\lgsi$ (line 8), and the while loop terminates when all the I-LGRs have $\lgsi\leq 0$, which occurs in less than $N_A$ iterations.
Since the bottleneck in the while loop is the recalculation of $\lgsi$'s which is $O(N_D^2N_A)$, the time complexity of Algorithm~\ref{alg:2v1assignment} is $O(N_D^2N_A^2)$.

% ALGORITHM 1v1:
 \begin{algorithm}[h]
 \caption{Assign 1v1 Defense \label{alg:1v1assignment}}
 \begin{small}
 \begin{algorithmic}[1]
\State Inputs: $\ateam_\text{assgn}$, $\dteam_\text{2v1}$, and $\dteam_\text{1v1}$ 
 \State $\ateam_\text{1v1}\gets \ateam \setminus \ateam_\text{assgn}$
\State Initialize a bipartite graph with $\{\dteam_\text{1v1},\dteam_\text{2v1}\}$ and $\ateam_\text{1v1}$
 \For{$k$ in $\dteam_\text{2v1}$}
     \If {Inequality in Eq.~\eqref{eq:ineligible} is satisfied}
    %  	\State Draw edges to intruders in the \implicit\ zone
     	\State Draw edges to $\forall\,A_j$ s.t. $\mf x_{A_j}\in\dwinr(D_R^k)\cap\dwinr(D_L^k)$
     \EndIf
 \EndFor
 \For{$D_i$ in $\dteam_\text{1v1}$}
    %  \State Draw edges to intruders in the defender winning region
     \State Draw edges to $\forall\,A_j$ s.t. $\mf x_{A_j}\in\dwinr(D_i)$
 \EndFor
 \State Solve maximum matching and save the edges for $\dteam_\text{1v1}$
 \State {\bf Return}: 1v1 assignments (edges for $\dteam_\text{1v1}$)
 \end{algorithmic}
 \end{small}
 \end{algorithm}
%
When assigning 1v1 games, Algorithm~\ref{alg:1v1assignment} accounts for the \implicit\ structure.
The implicit assignment is still applicable to the pairs in \sequential\ structure, but with a restriction.
Noting that each structure involves $n+1$ defenders and $n$ intruders, we can only consider one additional ``implicit'' assignment, otherwise there will be more intruders than the defenders.
To guarantee capture, it is necessary and sufficient for the additional intruder to be in the \implicit\ zone of the outermost defender pair (e.g., $(D_k,D_j)$ in Fig.~\ref{fig:sequential_2v1}).
In summary, a 2v1 defender pair, $\dboundary^k$, can have an \implicit\ if $D_R^k$ or $D_L^k$ are not used in any other 2v1 defense that is associated to a larger I-LGR, i.e.,
\bnl
n_D^k > n_D^m, \forall m\in \dteam_\text{2v1}\;\text{s.t.}, \dboundary^m\cap\dboundary^k\neq\emptyset
\label{eq:ineligible}
\enl

% Any intruder pair that does not satisfy this condition is eligible to have an implicit assignment.
The solution of the matching problem (line 9) only affects the behavior of the defenders in the set $\dteam_\text{1v1}$, but not the pairs in $\dteam_\text{2v1}$ because the assignments are only ``implicit'' for them.
This is why we only need the edges for $\dteam_\text{1v1}$.
The computational bottleneck in Algorithm~\ref{alg:1v1assignment} is the maximum matching, which is known to have efficient polynomial time algorithms \cite{Chen2017}.
Noting that $|\{\dteam_\text{1v1},\dteam_\text{2v1}\}|\leq N_D$ and $|\ateam_\text{1v1}|\leq N_A$, the number of nodes in the bipartite graph is at most $N_D+N_A$, which leads to $O((N_A+N_D)^w)$ time with $w<2.5$ \cite{Mucha2004}.
% The number of unique defenders involved in the 2v1 assignments, $N_D'$, is bounded by $|\dteam_\text{2v1}|\leq N_D'\leq 2|\dteam_\text{2v1}|$.



% % Figure: 
% \begin{figure}[t]
% \centering
% \includegraphics[width=.4\textwidth]
% {figures/assignment_example}
% \caption{
% }
% \label{fig:assignment_ex}
% \end{figure}
% %
% \todo{Use the figure in Simulation section to reduce space.}
Figure~\ref{fig:sim_example}a shows an example of the assignments given by Algorithm~\ref{alg:LGRdefense}.
Notice that a defender can have multiple 2v1 games assigned to it.
Algorithm~\ref{alg:2v1assignment} generated the \sequential\ structure involving $D_1,D_2,D_3$ and $D_4$.
% This is one of the main differences from the existing defense strategies (MM or MIS approach), and will be explained in detail in the next subsection.
%We will show that such overlapping assignments all require the same direction of motion from the defender, and will eventually dissolve into multiple 1v1 games.
% We will show that such overlapping assignments will eventually dissolve into multiple 1v1 games.
After the 2v1 assignments, $A_4$ and $A_5$ are left for 1v1 assignments.
The pair $(D_1,D_4)$ is eligible for the \implicit, and only $A_5$ is in the \implicit\ zone.
% Notice that intruder $A_5$ has no assignment at this time.
Therefore, the maximum matching in Algorithm~\ref{alg:1v1assignment} selects $A_4$ to be pursued by $D_5$ and leaves $A_5$ to be implicitly assigned to $(D_1,D_4)$.
% Another major difference from the existing defense policies is that, with our algorithm, even those intruders without explicit assignment at the current time can be shown to be captured when certain conditions are met.
% In fact, we will show in the next section that all intruders will be captured if $\Qest=0$ and $\lgsi_k\leq 1,\; \forall\, k$.
We will prove the performance guarantees in the remaining sections.



% Perfect defense
\subsection{Conditions for Perfect Defense} \label{sec:perfect_defense}
\noindent
This section finds the configuration for which the LGR defense (Algorithm~\ref{alg:LGRdefense}) achieves perfect defense: i.e., guarantees zero score $Q=0$.
%If a defender or a defender pair is assigned to a unique intruder, it is clear that the intruder is guaranteed to be captured.



\begin{lemma}\label{lem:completeness}
If $\Qest=0$ and $\lgsi_k\leq 1$, then no intruder is unmarked: i.e.,
each intruder has either (i) 1v1 assignment, (ii) 2v1 assignment, or (iii) implicit assignment.
% In other words, each intruder has one of the following: (i) one defender dedicated to perform 1v1 defense, (ii) a pair of defenders performing 2v1 defense with possible assignment to other 2v1 games, or (iii) a unique pair of defenders with implicit assignment structure.
\end{lemma}
\begin{proof}
It suffices to show that, after Algorithm~\ref{alg:2v1assignment}, the intruders without 2v1 assignment gets either 1v1 or implicit assignment.
We use Hall's marriage theorem \cite{Hall} to show that the maximum matching in Algorithm~\ref{alg:1v1assignment} covers all the intruders.
% Let $X$ denote the set of intruders without 2v1 assignment.
For any subset $W\subseteq \ateam_\text{1v1}$, let $\mc{N}(W)$ denote the neighbor set: i.e., the subset of defenders that can capture at least one in $W$.
Hall's theorem states that all intruders in $\ateam_\text{1v1}$ are covered if $|W|\leq |\mc{N}(W)|$ for all $W\subseteq \ateam_\text{1v1}$.

For $|W|=1$, it is easy to see by contradiction that every intruder has at least one edge:
if an intruder has no edge, then the smallest I-LGR that contains it will have $\lgsi \geq 1$,
% if an intruder has no edge, it implies that 
% there exists an I-LGR with $\lgsi=1$, 
which contradicts with the termination of Algorithm~\ref{alg:2v1assignment}.
% Similarly for $|W|=2$, suppose there exists a pair of intruders with only one defender node that has edges to them.
% It is easy to see that this configuration also leads to the existence of an I-LGR with $\lgsi=1$.

%We have proved $|W|\leq |\mc{N}(W)|$ is true for $|W|=1$ and 2.
%Now, to use mathematical induction, we suppose the above inequality is true for $|W|=1,..,n$ and prove that it guarantees the condition for $|W|=n+1$.
Now, suppose the inequality is true for $|W|=1,..,n$.
We will prove that the inequality is also true for $|W|=n+1$:
If the bipartite graph can be separated into $m$ connected components involving intruder subsets $w_1,.. w_m$, then we have $|\mc{N}(W)|=\sum_i^m |\mc{N}(w_i)|$ because the defender nodes for each subset $w_i$ are disjoint.
Since we have $|\mc{N}(w_i)|\geq |w_i|$ from the supposition that the inequality is true for $|w_i|\leq n$, we obtain $|\mc{N}(W)| \geq \sum_i^m |w_i| = |W|$.
If the bipartite graph is connected and $|\mc{N}(W)|\leq n$, there exists an I-LGR whose defender subteam is $\mc{N}(W)$ and the intruder subteam is $W$.
% Now suppose $|\mc{N}(W)|=n$.
Then this region has the score $\lgsi\geq(n+1)-n=1$.
Since this contradicts with the termination of Algorithm~\ref{alg:2v1assignment}, we obtain $|\mc{N}(W)|\geq n+1=|W|$.
% For the case where the bipartite graph is connected, suppose that $|\mc{N}(W)|=n$.
% There exists an I-LGR whose defender subteam is $\mc{N}(W)$ and the intruder subteam is $W$.
% This region has the score $\lgsi=(n+1)-n=1$, which again contradicts with the completeness of the 2v1 assignment.

With mathematical induction, we have shown that $|W|\leq |\mc{N}(W)|$ for $W\subseteq \ateam_\text{1v1}$ with any size.
Therefore, maximum matching in Algorithm~\ref{alg:1v1assignment} covers all the intruders.
\end{proof}


\begin{lemma}\label{lem:sequential_2v1noconflict}
If $\Qest=0$ and $\lgsi_k\leq1,\,\forall\,k$, then the \sequential\ structure generated by Algorithm~\ref{alg:2v1assignment} has no conflict (see Definition~\ref{def:conflict}).
% : all overlapping 2v1 assignments require the same direction of motion from each intruder.
%Suppose Algorithm~\ref{alg:2v1assignment} assigned multiple 2v1 games to $\di$.
%If $\Qest=0$ and $\lgsi_k\leq1,\,\forall\,k$, then all those assignments require the same direction of motion by $\di$.
\end{lemma}
\begin{proof}
%If $D_i$ serves as the left (or right) boundary defender for all of the 2v1 assignments, then the required motion is the same for all.
%We show by contradiction that $D_i$ does not serve as the left and right boundary defender simultaneously.
%
For $\di$ to have conflicting 2v1 assignments, the following condition is necessary: $\di$ has two I-LGRs, $l$ and $r$ with $\lgsi_l=\lgsi_r=1$, where $D_R^l = \di$ and $D_L^r=\di$.
If $D_i$ gets both assignments, then there is a conflict.
% : $l$ and $r$ denote the indices of the LGRs that $\di$ serves as the left and right boundary defender, with $q_l=q_r=0$ and $\lgsi_l=\lgsi_r=1$.

Consider $\awinri^m\triangleq\awinri(D_R^r,D_L^l)$, which contains both $\awinri^l$ and $\awinri^r$.
The score satisfies $\lgsi_m\geq (n_D^l+1)+(n_D^r+1)-(n_D^l+n_D^r+1)=1$.
% From the condition of the lemma, we know $\lgsi_m=1$.
We also know $\Qest=0 \Rightarrow q_m=0$, implying that $\dwinrp^m$ has at least one intruder to be assigned to $\dboundary^m$.
Since this assignment reduces one intruder from either $l$ or $r$, $\di$ only needs to perform 2v1 defense for one of the two: i.e., $\di$ does not get both assignments.
\end{proof}

\begin{lemma}\label{lem:sequential_2v1resolve}
If $\Qest=0$ and $\lgsi_k\leq1,\,\forall\,k$, then all \sequential\ structure given by Algorithm~\ref{alg:2v1assignment} turn into 1v1 games in finite time.
\end{lemma}
\begin{proof}
There are no conflicting 2v1 assignments, by Lemma~\ref{lem:sequential_2v1noconflict}.
Looking at each 2v1 game separately, the defender pair performs optimally against the intruder.
Recalling the 2v1 analysis, the intruder in $\dwinrp$ will eventually move into the defender winning region of either of the two boundary defenders (Prop.~\ref{prop:pincer}).
Every time such transition occurs, the number of interrelated 2v1 game decreases, and we have additional 1v1 and/or implicit assignment configuration.

Importantly, observe that the transition occurs by the intruder leaving an I-LGR and not by entering a new I-LGR, which implies that the local game scores $q$ and $\lgsi$ are both non-increasing.
Therefore, the condition $\Qest=0$ and $\lgsi_k\leq1$ will be preserved after the transition.
Since the conditions for no conflict (Lemma~\ref{lem:sequential_2v1noconflict}) are still true, the next transition that reduces the number of 2v1 games occurs in finite time.
Repeating this process, we see that the \sequential\ structure will separate into multiple 1v1 games and non-overlapping 2v1 games possibly having a implicit assignment structure.
With the result from Lemma~\ref{lem:unassigned_defense1}, the proof is completed.
\end{proof}


\begin{theorem}\label{thm:perfect_defence}
If the initial configuration is such that $\Qest=0$ and $\lgsi_k\leq 1, \forall\,k$, then the LGR-defense (Algorithm~\ref{alg:LGRdefense}) guarantees perfect defense.
\end{theorem}
\begin{proof}
By construction, the unique 1v1 and 2v1 assignments guarantee capture.
The \implicit\ and \sequential\ also guarantee capture by Lemmas \ref{lem:unassigned_defense1}~and~\ref{lem:sequential_2v1resolve}.
Since all intruders have either one of the above assignments (Lemma~\ref{lem:completeness}), the capture of all intruders is guaranteed.
%The in intruders is gutrude of allers have either (i) a unique 1v1 assignment, (ii) 2v1 assignment, or (iii) no assignment.
%By construction, every 1v1 assignment guarantees capture.
%Lemmas~\ref{lem:unassigned_defense1} and \ref{lem:unassigned_defense2} prove that intruders with no assignment will all be captured. 
%Lemma~\ref{lem:sequential_2v1} and the discussion that follows prove that all 2v1 assignments will lead to capture.
\end{proof}



% Saddle point equilibrium
\subsection{Saddle-point equilibrium}
\label{sec:saddle_point}
\noindent This section addresses the case when the intruder team can guarantee non-zero score: $\Qest>0$.
The idea behind the first line in Algorithm~\ref{alg:LGRdefense} is to ignore the intruders that cannot be captured, and make sure all other intruders are captured.
\begin{lemma}\label{lem:removal}
Suppose $\Qest=n>0$, then there exists a set of $n$ intruders whose removal will generate a new game with $\Qest=0$.
\end{lemma}
\begin{proof}
When $\Qest>0$, one can show by contradiction that there exists at least one intruder whose removal reduces $\Qest$ by $1$.
The contradiction is derived by supposing that there is no such intruder, and showing that it leads to the existence of $\djset$ with $\Qint(\djset)>\Qest$, which contradicts with the optimality of $\Qest$ in \eqref{eq:Qest}.

% Suppose there is no intruder whose removal reduces $\Qest$.
% Then we can show that there exists a selection of disjoint sets $G'$ such that $Q(G')>Q(G^*)=\Qest$ (details omitted for page constraints), which contradicts with the optimality of $\Qest$ and $G^*$.
% We have shown

% We show by contradiction that there exists an intruder whose removal decreases $\Qest$ by one.
% Suppose there is no such intruder.
% Then there exists at least two sets $\djset_1^*$ and $\djset_2^*$ that gives the optimal score $Q(\djset_1^*) = Q(\djset_2^*) = \Qest$, with the constraint $\subteam_A^k\cap\subteam_A^l=\emptyset$ for $k\in\djset_1^*$ and $l\in\djset_2^*$, i.e., no common intruders.
% The two sets do not share any intruder because if they did, then the removal of the common intruder will reduce both $Q(\djset_1^*)$ and $Q(\djset_2^*)$.

% Now, take $k\in\djset_1^*$ with $q_k>0$ and consider merging it to $\djset_2^*$.
% If $\awinrc^k\cap\awinrc^l=\emptyset$ for $\forall\, l\in\djset_2^*$, then $\djset_3 = \{k,\djset_2^*\}$ is a valid disjoint set and it has $Q(\djset_3)>Q(\djset_2^*)$, which contradicts with the optimality of $\djset_2^*$.
% If $k$ intersects with $l\in\djset_2^*$, then let $m$ be the smallest LGR that contains both $k$ and $l$.
% Since the regions intersect, we have $n_D^m<n_D^k+n_D^l$.
% However, since they share no intruders, we have $n_A^m\geq n_A^k+n_A^l$.
% Therefore, $q_m= n_A^m-n_D^m > n_A^k+n_A^l- n_D^k-n_D^l = q_k+q_l$, which again contradicts with the optimality of $\djset_2^*$.
% The case when $k$ intersects with multiple LGRs in $\djset_2^*$ can be treated similarly.

After removing one intruder, the same argument still holds if $\Qest$ is still positive.
Repeating this process, the score $\Qest$ reduces to zero after removing $n$ intruders.
% Also, observe that the order of the removal does not affect the result.
% Consider the optimally selected disjoint set $\mf G^*$.
% For an LGR with $q_k\geq 1$ in $\mf G^*$, we show by contradiction that there exists an intruder whose removal makes $q_i\leq q_k-1$ for all $i$ such that $\awinrc^i\subseteq\awinrc^k$; i.e., $\Qest$ is reduced by one.
% Suppose there is no such intruder.  
% Then we should have at least two LGRs $\awinrc^i$ and $\awinrc^j$ contained in $\awinrc^k$ that satisfy the following conditions: (i) $q_i=q_j=q_k$, and  (ii) $\subteam_A^i\cap\subteam_A^j=\emptyset$.
% If the two LGRs are disjoint, then $q_i+q_j = 2q_k > q_k$ contradicts with the assumption that $k\in G^*$ (we would have $i,j\in \mf G^*$ instead).  
% If the two LGRs intersect, let $\awinrc^m\subseteq \awinrc^k$ be the smallest LGR that contains both $\awinrc^i$ and $\awinrc^j$.
% One can show that this leads to a contradiction $q_m>q_k$.
% After removing one intruder, we can choose the next LGR in $\mf G^*$ with $q>0$ and repeat the process until $q_k\leq0,\,\forall\,k$.  Since each removed intruder contributes to the reduction in $\Qest$, at most $\Qest$ intruders need to be removed.
\end{proof}

Let $\aignore$ be a set of intruders with cardinality $|\aignore|=\Qest$, such that the removal of those intruders generate a new game with $\Qest=0$.
Following the proof of Lemma~\ref{lem:removal}, we can find $\aignore$ by visiting every intruder and asking whether it reduces $\Qest$ or not (Algorithm~\ref{alg:removal}).
Importantly, the answer remains the same whether $\Qest$ is already reduced or not.
Therefore, each intruder needs to be visited only once; Algorithm~\ref{alg:removal} terminates within less than $N_A$ iterations.
Since the bottleneck in the while loop is the computation of $\Qest$ (line 3), the time complexity is $O(N_AN_D^4)$.
% Every time the answer is yes, we remove that intruder from the game, and continue until $\Qest=0$.
% Assuming that the set $\djset^*$ is already known, the complexity is linear in $N_A$ since each intruder is visited only once.
% ALGORITHM:
\begin{algorithm}[h]
\caption{Removal of uncapturable intruders \label{alg:removal}}
\begin{small}
\begin{algorithmic}[1]
\State Initialize: $\aignore=\emptyset$, and $i=1$ 
\While {$\Qest>0$}
    \State $Q_{new}\gets$ compute $\Qest$ without $\{A_i,\aignore \}$
    \If {$Q_{new} < \Qest$}
        \State Append $A_i$ to $\aignore$
        \State $\Qest\gets Q_{new}$
    \EndIf
    \State $i\gets i+1$
\EndWhile
\State {\bf Return}: $\aignore$
\end{algorithmic}
\end{small}
\end{algorithm}
% \vspace{-10pt}


\begin{theorem}
If $\hat{q}_k\leq 1\,\forall\,k$ after removing $\Qest$ intruders found by Algorithm~\ref{alg:removal}, then the LGR-defense policy $\mf u_D^*$ guarantees
\bql
Q(\mf z_0; \mf u_D^*,\mf u_A)\leq  \Qest(\mf z_0), \; \forall \, \mf u_A\in U_A,
\label{eq:uDguarantee}
\eql
where $U_A$ is the set of all permissible intruder strategies.
\end{theorem}
\begin{proof}
The result immediately follows from Lemma~\ref{lem:removal} and Theorem~\ref{thm:perfect_defence}.
\end{proof}

Finally, the combination of the strategy $\mf u_A^*$ from Theorem~\ref{thm:Qlow} and $\mf u_D^*$ from Theorem~\ref{thm:perfect_defence} gives us the following result:
\begin{corollary}
If $\hat{q}_k\leq 1\,\forall\,k$ after removing $\Qest$ intruders found by Algorithm~\ref{alg:removal}, then
\bql
Q(\mf u_D^*,\mf u_A)\leq  Q(\mf u_D^*,\mf u_A^*) \leq Q(\mf u_D,\mf u_A^*),
\eql
i.e., the strategies $(\mf u_D^*,\mf u_A^*)$ are at a saddle-point equilibrium, and the value of the game is $Q^*(\mf z_0) = \Qest(\mf z_0)$.
\end{corollary}
If the intruders stick to $\mf u_A^*$, then the defender team cannot reduce the score by changing their strategy.
Similarly, if the defenders keep $\mf u_D^*$, then the intruders cannot increase the score by changing their strategy.
% This result indicates the optimality of the proposed strategy in the sense that any deviation does not improve the score as long as the opponent sticks to the equilibrium strategy.


==> defense_policy.tex <==
\section{The LGR Defense Policy \label{sec:defense_policy}}

\noindent This section proposes the defender team strategy (LGR-defense strategy) that outperforms the existing MM and MIS policies.
%We first present the algorithm and then prove the condition when all intruders are captured.
We first discuss special multi-player engagements that our policy leverages.
We then present the LGR-defense algorithm and prove its performance guarantees.
Finally, we show that the score is bounded from above by $\Qest$ under a certain condition, indicating that $\Qest$ is the exact outcome (equilibrium solution) of the game.

 
\subsection{Extended Engagement Types}
\noindent 
We discuss two additional types of engagements that appear in the LGR-defense: the \emph{\implicit} and the \emph{\sequential}.
% This section discusses complex multi-player configurations that can be analyzed using the 1v1 and 2v1 building blocks.
Although these engagements will be analyzed using the 1v1 and 2v1 building blocks, the distinct feature is the aspect of dynamically changing assignments which the existing MM and MIS approaches fail to capture.
We will show that there exists a ``greedy'' behavior that only considers current configuration, and yet performs optimally over the entire game duration.

\begin{definition}
The \emph{\textbf{\implicit}} structure is a two vs.\ two engagement where the defender pair is assigned to one intruder in $\dwinrp(i,j)$, but there is another intruder in $\dwinr(i)\cap\dwinr(j)$, defined as the \implicit\ zone.
\end{definition}
% Figure: unassigned defense
\begin{figure}[t]
\centering
\includegraphics[width=.48\textwidth]
{figures/unassigned_defense}
\caption{The \implicit\ structure.
(a) Initial configuration where $A_1$ has 2v1 assignment, and $A_2$ is in the \implicit~zone.
(b) The structure is resolved into two 1v1 assignments.
}
\label{fig:unassigned_defense}
\vspace{-10pt}
\end{figure}
%
See Fig~\ref{fig:unassigned_defense}a for an example.
First note that MM assignment would ignore $A_1$ since it is not capturable by any individual defender.
The MIS assignment chooses from assigning (i) the pair to $A_1$, or (ii) one defender to $A_2$ (same as MM), but cannot have both because one of the defenders will have overlapping assignments.
Importantly, the two choices are equally good in the MIS analysis since they both guarantee one capture.
What MIS fails to see is that assigning the pair to $A_1$ is the optimal choice here, and in fact it leads to the capture of both intruders:
%Suppose the defenders are performing 2v1 against A1, and A2 is ignored for now.
%Algorithm~\ref{alg:LGRdefense} assigns the pair ($\di,\dj$) to $A_1$, but no defender to $A_2$ because there is no free defender for the 1v1 assignment nor it is in $\dwinrp(i,j)$ for the 2v1 assignment.
%Nevertheless, the intruder in this position will eventually get a unique 1v1 assignment.

\begin{lemma}\label{lem:unassigned_defense1}
The \emph{\implicit} structure will turn into two 1v1 assignments in finite time.
\end{lemma}
\begin{proof}
From the 2v1 assignment against $A_1$, $\di$ moves ccw and $\dj$ moves cw.
Under this movement, $A_2$ remains in $\dwinr(i)\cap\dwinr(j)$ because it cannot penetrate $\di$'s left barrier nor $\dj$'s right barrier (Prop.~\ref{prop:1v1barrier}).
Before they meet at the midpoint, $A_1$ will move into either $\dwinr(i)$ or $\dwinr(j)$ (Prop.~\ref{prop:pincer}).
Suppose without the loss of generality $\mf x_{A_1}\in \dwinr(i)$, then $A_2$ will get 1v1 assignment to $\dj$. 
\end{proof}

We use the term ``implicit'' to highlight the fact that no defender is ``explicitly'' assigned to $A_2$.
Nevertheless, the greedy behavior against $A_1$ guarantees the capture of $A_2$ as well.
The second structure (i.e., a combination of configuration and assignment) is defined next:

\begin{definition}
The \emph{\textbf{\sequential}} structure is an $n+1$ vs.\ $n$ engagement generated by $n$ interrelated 2v1 games with overlapping defenders.
\end{definition}

% Figure: sequential 2v1
\begin{figure}[t]
\centering
\includegraphics[width=.48\textwidth]
{figures/sequential_2v1}
\caption{
Sequential 2v1 structure with $n=2$.
(a) The defender $D_j$ has two 2v1 assignments, and cw motion is required for both.
(b) The structure is resolved into two 1v1 assignments.
}
\label{fig:sequential_2v1}
\end{figure}
%

Fig.~\ref{fig:sequential_2v1}a shows the simplest example of such configuration.
Note that we are now considering an assignment that is prohibited in the MIS formulation; defender $D_j$ has two 2v1 games assigned to it.
Also note that, by definition, each defender pair can have at most one intruder assigned to it (otherwise, it will not be $n+1$ vs. $n$).
The key concept to analyze the success in this configuration is defined next:

\begin{definition}
The overlapping 2v1 assignments are \emph{\textbf{conflicting}} if they require opposing (cw and ccw) direction of motion from the defender.
\label{def:conflict}
\end{definition}

For example, $D_j$ in Fig.~\ref{fig:sequential_2v1}a has non-conflicting assignments, because the two assignments both require cw motion.
Despite the overlap, it can behave optimally for both $A_1$ and $A_2$, which leads to the resolved configuration in Fig.~\ref{fig:sequential_2v1}b.
We formally show in Sec.~\ref{sec:perfect_defense} that the \sequential\ leads to the capture of all intruders if they are non-conflicting.
The defense algorithm that leverages these engagement types is introduced next.
% We defer the detailed discussions and the performance guarantees to Sec.~\ref{sec:perfect_defense}
%Each defender pair has at most one intruder assigned to it, but the individual defender may have more than one 2v1 games assigned to it.
%Fig.~\ref{fig:sequential_2v1}a shows the simplest example of such configuration.
%Three defenders are interrelated through the pairing for the cooperative defense.
%Defender $D_j$ has two 2v1 games assigned to it, which was prohibited in the MIS algorithm.
%\begin{lemma}
%If the overlapping assignments demand the same direction of motion for each defender, then the \sequential structure will turn into 1v1 assignments in finite time.
%\end{lemma}
%\begin{proof}
%Looking at each 2v1 game separately, the defender pair is performing optimally against the intruder.
%Recalling the 2v1 analysis, the intruder in $\dwinrp$ will eventually move into the defender winning region of either of the two boundary defenders (Property~\ref{}).
%Every time such transition occurs, the number of interrelated 2v1 game decreases, and we have additional 1v1 and/or implicit assignment configuration.
%\end{proof}



\subsection{The LGR-defense Algorithm}
\noindent
% Our algorithm visits each intruder once and decides a defender or a defender pair to be assigned to it.
% To narrow down the selection of the defender for a given intruder, we identify a unique I-LGR for each intruder as follows.
We first extend the concept of LGS defined for LGRs in Lemma~\ref{lem:lgs} to I-LGRs.
The \emph{independent local game score} (I-LGS) is defined as
\begin{gather}
\lgsi_k \triangleq \hat{n}_A^k - n_D^k =  q_k + \Delta n_A^k,
\end{gather}
where $\Delta n_A^k$ is the number of intruders in the paired defense region $\dwinrp^k$.

The local game score of $q_k=0$ was a critical number in Sec.~\ref{sec:QLG} since it meant that any additional intruder in the LGR will immediately lead to a positive intruder score (Lemma~\ref{lem:lgs}). 
% We say that $k$th LGR (resp.~I-LGR) is \emph{occupied} if $q_k\geq 0$ (resp.~$\lgsi_k\geq 0$): every defender in the region needs to capture one intruder to avoid intrusion.
% We say that $k$th LGR is \emph{occupied} if $q_k\geq 0$: every defender in the LGR needs to capture one intruder to avoid intrusion.
The I-LGS has another critical number: $\lgsi_k=1$.
Unlike $q_k=1$, this configuration does not immediately lead to intruder score; suppose $q_k \leq 0$ and $\lgsi_k = 1$, then one intruder in $\dwinrp^k$ can be captured by the pincer maneuver of the boundary defenders, and the rest may be captured by the defender subteam $\subteam_D^k$.
What $\lgsi_k=1$ immediately tells us is that the boundary defenders $(D_R^k,D_L^k)$ need to perform a pincer maneuver.
Otherwise the intruder in $\dwinrp^k$ can enter $\awinrc^k$ to achieve $q_k>0$, which guarantees a score.

% ALGORITHM
\begin{algorithm}[t]
\caption{LGR Defense \label{alg:LGRdefense}}
\begin{small}
\begin{algorithmic}[1]
\State Remove uncapturable intruders using Algorithm~\ref{alg:removal}
\State Assign 2v1 defense using Algorithm~\ref{alg:2v1assignment}
\State Assign 1v1 defense using Algorithm~\ref{alg:1v1assignment}
\State {\bf Return}: assignments (i.e., direction of motion)
\end{algorithmic}
\end{small}
\end{algorithm}
% 
The LGR defense strategy is presented in Algorithm~\ref{alg:LGRdefense}.
It is continuously run throughout the game to update the defender-intruder assignments that uniquely define each defender's direction of motion.
In the first line, the intruders that are guaranteed to score are ignored so that the defenders can focus on the rest (to be discussed in Sec.~\ref{sec:saddle_point}).
The cooperative 2v1 defense and the individual 1v1 defense are considered sequentially.
To simplify the proofs in the sequel, we restrict ourselves to the case when $\lgsi_k\leq 1,\,\forall\,k$ after the removal of uncapturable intruders (although we empirically observe that the algorithm handles general case).


% ALGORITHM:
 \begin{algorithm}[t]
 \caption{Assign 2v1 Defense \label{alg:2v1assignment}}
 \begin{small}
 \begin{algorithmic}[1]
\State Initialize: $\mf A_\text{assgn}=\emptyset$, $\mf D_\text{2v1}=\emptyset$, and $\mf D_\text{1v1}=\dteam$
 \While{$\exists\,k$ s.t. $\lgsi_k \geq 1$}
\State $m \gets \argmax_k n_D^k$ for $k$ s.t. $\lgsi_k \geq 1$
     \State $A_j \gets$ select one intruder in $\dwinrp^m$
    %  \State Assign $A_j$ to the pair ($D_R^m,D_L^m$)
     \State Append $A_j$ to $\mf A_\text{assgn}$, and $m$ to $\mf D_\text{2v1}$
     \State Remove $D_R^m$ and $D_L^m$ from $\mf D_\text{1v1}$
     \State Recompute $\lgsi_k$ for all $k$ with $\ateam \setminus \mf A_\text{assgn}$
 \EndWhile
\State {\bf Return}: $\mf D_\text{2v1}$, $\mf D_\text{1v1}$ and $\mf A_\text{assgn}$
 \end{algorithmic}
 \end{small}
 \end{algorithm}
%
The assignment of cooperative 2v1 games is presented in Algorithm~\ref{alg:2v1assignment}.
The I-LGRs with $\lgsi=1$ are visited sequentially from the largest to the smallest in terms of the subteam size.
In each iteration, one intruder in $\dwinrp$ is assigned to the boundary defenders (line 5) regardless of whether the defenders already have other 2v1 assignments or not, which potentially generates the \sequential\ structure.
The indices saved in $\dteam_\text{2v1}$ is sufficient to know which defender should perform a pincer movement with which pair.
The already assigned intruders are removed from the computation of $\lgsi$ (line 8), and the while loop terminates when all the I-LGRs have $\lgsi\leq 0$, which occurs in less than $N_A$ iterations.
Since the bottleneck in the while loop is the recalculation of $\lgsi$'s which is $O(N_D^2N_A)$, the time complexity of Algorithm~\ref{alg:2v1assignment} is $O(N_D^2N_A^2)$.

When assigning 1v1 games, Algorithm~\ref{alg:1v1assignment} accounts for the \implicit\ structure.
The implicit assignment is still applicable to the pairs in \sequential\ structure, but with a restriction.
Noting that each structure involves $n+1$ defenders and $n$ intruders, we can only consider one additional ``implicit'' assignment, otherwise there will be more intruders than the defenders.
To guarantee capture, it is necessary and sufficient for the additional intruder to be in the \implicit\ zone of the outermost defender pair (e.g., $(D_k,D_j)$ in Fig.~\ref{fig:sequential_2v1}).
% We consider this by disqualifying a 2v1 defender pair, $\dboundary^k$, from having an \implicit\ if it satisfies the following condition:
% \bnl
% \begin{array}{l}
% (a)\; \exists\,m \text{\;with\;}\lgsi_m=1,\;\text{s.t.,}\;  \dboundary^k\cap\dboundary^m\neq\emptyset \text{\; and} \\
% (b)\; n_D^m > n_D^k.
% \end{array}
% \label{eq:ineligible}
% \enl
In summary, a 2v1 defender pair, $\dboundary^k$, can have an \implicit\ if $D_R^k$ or $D_L^k$ are not used in any other 2v1 defense that is associated to a larger I-LGR, i.e.,
% \begin{itemize}
%     \item[(a)] It does not share a defender with other 2v1 defenses; and
%     \item[(b)] It shares a defender with other 2v1 defenses, but 
% \end{itemize}
% \bnl
% \begin{array}{l}
% \text{$D_R^k$ or $D_L^k$ are not used in any other 2v1 defense}\\
% \text{that is associated to a larger I-LGR,}
% (a)\; \text{There is no overlapping assignment;} \text{\; or} \\
% (b)\; \text{Overlap with $\dboundary^m$,} \text{\;but\;} n_D^m < n_D^k.
% \end{array}
% \label{eq:ineligible}
% \enl
\bnl
n_D^k > n_D^m, \forall m\in \dteam_\text{2v1}\;\text{s.t.}, \dboundary^m\cap\dboundary^k\neq\emptyset
\label{eq:ineligible}
\enl

% Any intruder pair that does not satisfy this condition is eligible to have an implicit assignment.
The solution of the matching problem (line 9) only affects the behavior of the defenders in the set $\dteam_\text{1v1}$, but not the pairs in $\dteam_\text{2v1}$ because the assignments are only ``implicit'' for them.
This is why we only need the edges for $\dteam_\text{1v1}$.
The computational bottleneck in Algorithm~\ref{alg:1v1assignment} is the maximum matching, which is known to have efficient polynomial time algorithms \cite{Chen2017}.
Noting that $|\{\dteam_\text{1v1},\dteam_\text{2v1}\}|\leq N_D$ and $|\ateam_\text{1v1}|\leq N_A$, the number of nodes in the bipartite graph is at most $N_D+N_A$, which leads to $O((N_A+N_D)^w)$ time with $w<2.5$ \cite{Mucha2004}.
% The number of unique defenders involved in the 2v1 assignments, $N_D'$, is bounded by $|\dteam_\text{2v1}|\leq N_D'\leq 2|\dteam_\text{2v1}|$.

% ALGORITHM 1v1:
 \begin{algorithm}[t]
 \caption{Assign 1v1 Defense \label{alg:1v1assignment}}
 \begin{small}
 \begin{algorithmic}[1]
\State Inputs: $\ateam_\text{assgn}$, $\dteam_\text{2v1}$, and $\dteam_\text{1v1}$ 
 \State $\ateam_\text{1v1}\gets \ateam \setminus \ateam_\text{assgn}$
\State Initialize a bipartite graph with $\{\dteam_\text{1v1},\dteam_\text{2v1}\}$ and $\ateam_\text{1v1}$
 \For{$k$ in $\dteam_\text{2v1}$}
     \If {Inequality in Eq.~\eqref{eq:ineligible} is satisfied}
    %  	\State Draw edges to intruders in the \implicit\ zone
     	\State Draw edges to $\forall\,A_j$ s.t. $\mf x_{A_j}\in\dwinr(D_R^k)\cap\dwinr(D_L^k)$
     \EndIf
 \EndFor
 \For{$D_i$ in $\dteam_\text{1v1}$}
    %  \State Draw edges to intruders in the defender winning region
     \State Draw edges to $\forall\,A_j$ s.t. $\mf x_{A_j}\in\dwinr(D_i)$
 \EndFor
 \State Solve maximum matching and save the edges for $\dteam_\text{1v1}$
 \State {\bf Return}: 1v1 assignments (edges for $\dteam_\text{1v1}$)
 \end{algorithmic}
 \end{small}
 \end{algorithm}
%


% % Figure: 
% \begin{figure}[t]
% \centering
% \includegraphics[width=.4\textwidth]
% {figures/assignment_example}
% \caption{
% }
% \label{fig:assignment_ex}
% \end{figure}
% %
% \todo{Use the figure in Simulation section to reduce space.}
Figure~\ref{fig:sim_example}a shows an example of the assignments given by Algorithm~\ref{alg:LGRdefense}.
Notice that a defender can have multiple 2v1 games assigned to it.
Algorithm~\ref{alg:2v1assignment} generated the \sequential\ structure involving $D_1,D_2,D_3$ and $D_4$.
% This is one of the main differences from the existing defense strategies (MM or MIS approach), and will be explained in detail in the next subsection.
%We will show that such overlapping assignments all require the same direction of motion from the defender, and will eventually dissolve into multiple 1v1 games.
% We will show that such overlapping assignments will eventually dissolve into multiple 1v1 games.
After the 2v1 assignments, $A_4$ and $A_5$ are left for 1v1 assignments.
The pair $(D_1,D_4)$ is eligible for the \implicit, and only $A_5$ is in the \implicit\ zone.
% Notice that intruder $A_5$ has no assignment at this time.
Therefore, the maximum matching in Algorithm~\ref{alg:1v1assignment} selects $A_4$ to be pursued by $D_5$ and leaves $A_5$ to be implicitly assigned to $(D_1,D_4)$.
% Another major difference from the existing defense policies is that, with our algorithm, even those intruders without explicit assignment at the current time can be shown to be captured when certain conditions are met.
% In fact, we will show in the next section that all intruders will be captured if $\Qest=0$ and $\lgsi_k\leq 1,\; \forall\, k$.
We will prove the performance guarantees in the remaining sections.



% Perfect defense
\subsection{Conditions for Perfect Defense} \label{sec:perfect_defense}
\noindent
This section finds the configuration for which the LGR defense (Algorithm~\ref{alg:LGRdefense}) achieves perfect defense: i.e., guarantees zero score $Q=0$.
%If a defender or a defender pair is assigned to a unique intruder, it is clear that the intruder is guaranteed to be captured.



\begin{lemma}\label{lem:completeness}
If $\Qest=0$ and $\lgsi_k\leq 1$, then no intruder is unmarked: i.e.,
each intruder has either (i) 1v1 assignment, (ii) 2v1 assignment, or (iii) implicit assignment.
% In other words, each intruder has one of the following: (i) one defender dedicated to perform 1v1 defense, (ii) a pair of defenders performing 2v1 defense with possible assignment to other 2v1 games, or (iii) a unique pair of defenders with implicit assignment structure.
\end{lemma}
\begin{proof}
It suffices to show that, after Algorithm~\ref{alg:2v1assignment}, the intruders without 2v1 assignment gets either 1v1 or implicit assignment.
We use Hall's marriage theorem \cite{Hall} to show that the maximum matching in Algorithm~\ref{alg:1v1assignment} covers all the intruders.
% Let $X$ denote the set of intruders without 2v1 assignment.
For any subset $W\subseteq \ateam_\text{1v1}$, let $\mc{N}(W)$ denote the neighbor set: i.e., the subset of defenders that can capture at least one in $W$.
Hall's theorem states that all intruders in $\ateam_\text{1v1}$ are covered if $|W|\leq |\mc{N}(W)|$ for all $W\subseteq \ateam_\text{1v1}$.

For $|W|=1$, it is easy to see by contradiction that every intruder has at least one edge:
if an intruder has no edge, then the smallest I-LGR that contains it will have $\lgsi \geq 1$,
% if an intruder has no edge, it implies that 
% there exists an I-LGR with $\lgsi=1$, 
which contradicts with the termination of Algorithm~\ref{alg:2v1assignment}.
% Similarly for $|W|=2$, suppose there exists a pair of intruders with only one defender node that has edges to them.
% It is easy to see that this configuration also leads to the existence of an I-LGR with $\lgsi=1$.

%We have proved $|W|\leq |\mc{N}(W)|$ is true for $|W|=1$ and 2.
%Now, to use mathematical induction, we suppose the above inequality is true for $|W|=1,..,n$ and prove that it guarantees the condition for $|W|=n+1$.
Now, suppose the inequality is true for $|W|=1,..,n$.
We will prove that the inequality is also true for $|W|=n+1$:
If the bipartite graph can be separated into $m$ connected components involving intruder subsets $w_1,.. w_m$, then we have $|\mc{N}(W)|=\sum_i^m |\mc{N}(w_i)|$ because the defender nodes for each subset $w_i$ are disjoint.
Since we have $|\mc{N}(w_i)|\geq |w_i|$ from the supposition that the inequality is true for $|w_i|\leq n$, we obtain $|\mc{N}(W)| \geq \sum_i^m |w_i| = |W|$.
If the bipartite graph is connected and $|\mc{N}(W)|\leq n$, there exists an I-LGR whose defender subteam is $\mc{N}(W)$ and the intruder subteam is $W$.
% Now suppose $|\mc{N}(W)|=n$.
Then this region has the score $\lgsi\geq(n+1)-n=1$.
Since this contradicts with the termination of Algorithm~\ref{alg:2v1assignment}, we obtain $|\mc{N}(W)|\geq n+1=|W|$.
% For the case where the bipartite graph is connected, suppose that $|\mc{N}(W)|=n$.
% There exists an I-LGR whose defender subteam is $\mc{N}(W)$ and the intruder subteam is $W$.
% This region has the score $\lgsi=(n+1)-n=1$, which again contradicts with the completeness of the 2v1 assignment.

With mathematical induction, we have shown that $|W|\leq |\mc{N}(W)|$ for $W\subseteq \ateam_\text{1v1}$ with any size.
Therefore, maximum matching in Algorithm~\ref{alg:1v1assignment} covers all the intruders.
\end{proof}


\begin{lemma}\label{lem:sequential_2v1noconflict}
If $\Qest=0$ and $\lgsi_k\leq1,\,\forall\,k$, then the \sequential\ structure generated by Algorithm~\ref{alg:2v1assignment} has no conflict (see Definition~\ref{def:conflict}).
% : all overlapping 2v1 assignments require the same direction of motion from each intruder.
%Suppose Algorithm~\ref{alg:2v1assignment} assigned multiple 2v1 games to $\di$.
%If $\Qest=0$ and $\lgsi_k\leq1,\,\forall\,k$, then all those assignments require the same direction of motion by $\di$.
\end{lemma}
\begin{proof}
%If $D_i$ serves as the left (or right) boundary defender for all of the 2v1 assignments, then the required motion is the same for all.
%We show by contradiction that $D_i$ does not serve as the left and right boundary defender simultaneously.
%
For $\di$ to have conflicting 2v1 assignments, the following condition is necessary: $\di$ has two I-LGRs, $l$ and $r$ with $\lgsi_l=\lgsi_r=1$, where $D_R^l = \di$ and $D_L^r=\di$.
If $D_i$ gets both assignments, then there is a conflict.
% : $l$ and $r$ denote the indices of the LGRs that $\di$ serves as the left and right boundary defender, with $q_l=q_r=0$ and $\lgsi_l=\lgsi_r=1$.

Consider $\awinri^m\triangleq\awinri(D_R^r,D_L^l)$, which contains both $\awinri^l$ and $\awinri^r$.
The score satisfies $\lgsi_m\geq (n_D^l+1)+(n_D^r+1)-(n_D^l+n_D^r+1)=1$.
% From the condition of the lemma, we know $\lgsi_m=1$.
We also know $\Qest=0 \Rightarrow q_m=0$, implying that $\dwinrp^m$ has at least one intruder to be assigned to $\dboundary^m$.
Since this assignment reduces one intruder from either $l$ or $r$, $\di$ only needs to perform 2v1 defense for one of the two: i.e., $\di$ does not get both assignments.
\end{proof}

\begin{lemma}\label{lem:sequential_2v1resolve}
If $\Qest=0$ and $\lgsi_k\leq1,\,\forall\,k$, then all \sequential\ structure given by Algorithm~\ref{alg:2v1assignment} turn into 1v1 games in finite time.
\end{lemma}
\begin{proof}
There are no conflicting 2v1 assignments, by Lemma~\ref{lem:sequential_2v1noconflict}.
Looking at each 2v1 game separately, the defender pair performs optimally against the intruder.
Recalling the 2v1 analysis, the intruder in $\dwinrp$ will eventually move into the defender winning region of either of the two boundary defenders (Prop.~\ref{prop:pincer}).
Every time such transition occurs, the number of interrelated 2v1 game decreases, and we have additional 1v1 and/or implicit assignment configuration.

Importantly, observe that the transition occurs by the intruder leaving an I-LGR and not by entering a new I-LGR, which implies that the local game scores $q$ and $\lgsi$ are both non-increasing.
Therefore, the condition $\Qest=0$ and $\lgsi_k\leq1$ will be preserved after the transition.
Since the conditions for no conflict (Lemma~\ref{lem:sequential_2v1noconflict}) are still true, the next transition that reduces the number of 2v1 games occurs in finite time.
Repeating this process, we see that the \sequential\ structure will separate into multiple 1v1 games and non-overlapping 2v1 games possibly having a implicit assignment structure.
With the result from Lemma~\ref{lem:unassigned_defense1}, the proof is completed.
\end{proof}


\begin{theorem}\label{thm:perfect_defence}
If the initial configuration is such that $\Qest=0$ and $\lgsi_k\leq 1, \forall\,k$, then the LGR-defense (Algorithm~\ref{alg:LGRdefense}) guarantees perfect defense.
\end{theorem}
\begin{proof}
By construction, the unique 1v1 and 2v1 assignments guarantee capture.
The \implicit\ and \sequential\ also guarantee capture by Lemmas \ref{lem:unassigned_defense1}~and~\ref{lem:sequential_2v1resolve}.
Since all intruders have either one of the above assignments (Lemma~\ref{lem:completeness}), the capture of all intruders is guaranteed.
%The in intruders is gutrude of allers have either (i) a unique 1v1 assignment, (ii) 2v1 assignment, or (iii) no assignment.
%By construction, every 1v1 assignment guarantees capture.
%Lemmas~\ref{lem:unassigned_defense1} and \ref{lem:unassigned_defense2} prove that intruders with no assignment will all be captured. 
%Lemma~\ref{lem:sequential_2v1} and the discussion that follows prove that all 2v1 assignments will lead to capture.
\end{proof}



% Saddle point equilibrium
\subsection{Saddle-point equilibrium}
\label{sec:saddle_point}
\noindent This section addresses the case when the intruder team can guarantee non-zero score: $\Qest>0$.
The idea behind the first line in Algorithm~\ref{alg:LGRdefense} is to ignore the intruders that cannot be captured, and make sure all other intruders are captured.
\begin{lemma}\label{lem:removal}
Suppose $\Qest=n>0$, then there exists a set of $n$ intruders whose removal will generate a new game with $\Qest=0$.
\end{lemma}
\begin{proof}
When $\Qest>0$, one can show by contradiction that there exists at least one intruder whose removal reduces $\Qest$ by $1$.
The contradiction is derived by supposing that there is no such intruder, and showing that it leads to the existence of $\djset$ with $\Qint(\djset)>\Qest$, which contradicts with the optimality of $\Qest$ in \eqref{eq:Qest}.

% Suppose there is no intruder whose removal reduces $\Qest$.
% Then we can show that there exists a selection of disjoint sets $G'$ such that $Q(G')>Q(G^*)=\Qest$ (details omitted for page constraints), which contradicts with the optimality of $\Qest$ and $G^*$.
% We have shown

% We show by contradiction that there exists an intruder whose removal decreases $\Qest$ by one.
% Suppose there is no such intruder.
% Then there exists at least two sets $\djset_1^*$ and $\djset_2^*$ that gives the optimal score $Q(\djset_1^*) = Q(\djset_2^*) = \Qest$, with the constraint $\subteam_A^k\cap\subteam_A^l=\emptyset$ for $k\in\djset_1^*$ and $l\in\djset_2^*$, i.e., no common intruders.
% The two sets do not share any intruder because if they did, then the removal of the common intruder will reduce both $Q(\djset_1^*)$ and $Q(\djset_2^*)$.

% Now, take $k\in\djset_1^*$ with $q_k>0$ and consider merging it to $\djset_2^*$.
% If $\awinrc^k\cap\awinrc^l=\emptyset$ for $\forall\, l\in\djset_2^*$, then $\djset_3 = \{k,\djset_2^*\}$ is a valid disjoint set and it has $Q(\djset_3)>Q(\djset_2^*)$, which contradicts with the optimality of $\djset_2^*$.
% If $k$ intersects with $l\in\djset_2^*$, then let $m$ be the smallest LGR that contains both $k$ and $l$.
% Since the regions intersect, we have $n_D^m<n_D^k+n_D^l$.
% However, since they share no intruders, we have $n_A^m\geq n_A^k+n_A^l$.
% Therefore, $q_m= n_A^m-n_D^m > n_A^k+n_A^l- n_D^k-n_D^l = q_k+q_l$, which again contradicts with the optimality of $\djset_2^*$.
% The case when $k$ intersects with multiple LGRs in $\djset_2^*$ can be treated similarly.

After removing one intruder, the same argument still holds if $\Qest$ is still positive.
Repeating this process, the score $\Qest$ reduces to zero after removing $n$ intruders.
% Also, observe that the order of the removal does not affect the result.
% Consider the optimally selected disjoint set $\mf G^*$.
% For an LGR with $q_k\geq 1$ in $\mf G^*$, we show by contradiction that there exists an intruder whose removal makes $q_i\leq q_k-1$ for all $i$ such that $\awinrc^i\subseteq\awinrc^k$; i.e., $\Qest$ is reduced by one.
% Suppose there is no such intruder.  
% Then we should have at least two LGRs $\awinrc^i$ and $\awinrc^j$ contained in $\awinrc^k$ that satisfy the following conditions: (i) $q_i=q_j=q_k$, and  (ii) $\subteam_A^i\cap\subteam_A^j=\emptyset$.
% If the two LGRs are disjoint, then $q_i+q_j = 2q_k > q_k$ contradicts with the assumption that $k\in G^*$ (we would have $i,j\in \mf G^*$ instead).  
% If the two LGRs intersect, let $\awinrc^m\subseteq \awinrc^k$ be the smallest LGR that contains both $\awinrc^i$ and $\awinrc^j$.
% One can show that this leads to a contradiction $q_m>q_k$.
% After removing one intruder, we can choose the next LGR in $\mf G^*$ with $q>0$ and repeat the process until $q_k\leq0,\,\forall\,k$.  Since each removed intruder contributes to the reduction in $\Qest$, at most $\Qest$ intruders need to be removed.
\end{proof}

Let $\aignore$ be a set of intruders with cardinality $|\aignore|=\Qest$, such that the removal of those intruders generate a new game with $\Qest=0$.
Following the proof of Lemma~\ref{lem:removal}, we can find $\aignore$ by visiting every intruder and asking whether it reduces $\Qest$ or not (Algorithm~\ref{alg:removal}).
Importantly, the answer remains the same whether $\Qest$ is already reduced or not.
Therefore, each intruder needs to be visited only once; Algorithm~\ref{alg:removal} terminates within less than $N_A$ iterations.
Since the bottleneck in the while loop is the computation of $\Qest$ (line 3), the time complexity is $O(N_AN_D^4)$.
% Every time the answer is yes, we remove that intruder from the game, and continue until $\Qest=0$.
% Assuming that the set $\djset^*$ is already known, the complexity is linear in $N_A$ since each intruder is visited only once.
% ALGORITHM:
\begin{algorithm}[t]
\caption{Removal of uncapturable intruders \label{alg:removal}}
\begin{small}
\begin{algorithmic}[1]
\State Initialize: $\aignore=\emptyset$, and $i=1$ 
\While {$\Qest>0$}
    \State $Q_{new}\gets$ compute $\Qest$ without $\{A_i,\aignore \}$
    \If {$Q_{new} < \Qest$}
        \State Append $A_i$ to $\aignore$
        \State $\Qest\gets Q_{new}$
    \EndIf
    \State $i\gets i+1$
\EndWhile
\State {\bf Return}: $\aignore$
\end{algorithmic}
\end{small}
\end{algorithm}
% \vspace{-10pt}


\begin{theorem}
If $\hat{q}_k\leq 1\,\forall\,k$ after removing $\Qest$ intruders found by Algorithm~\ref{alg:removal}, then the LGR-defense policy $\mf u_D^*$ guarantees
\bql
Q(\mf z_0; \mf u_D^*,\mf u_A)\leq  \Qest(\mf z_0), \; \forall \, \mf u_A\in U_A,
\label{eq:uDguarantee}
\eql
where $U_A$ is the set of all permissible intruder strategies.
\end{theorem}
\begin{proof}
The result immediately follows from Lemma~\ref{lem:removal} and Theorem~\ref{thm:perfect_defence}.
\end{proof}

Finally, the combination of the strategy $\mf u_A^*$ from Theorem~\ref{thm:Qlow} and $\mf u_D^*$ from Theorem~\ref{thm:perfect_defence} gives us the following result:
\begin{corollary}
If $\hat{q}_k\leq 1\,\forall\,k$ after removing $\Qest$ intruders found by Algorithm~\ref{alg:removal}, then
\bql
Q(\mf u_D^*,\mf u_A)\leq  Q(\mf u_D^*,\mf u_A^*) \leq Q(\mf u_D,\mf u_A^*),
\eql
i.e., the strategies $(\mf u_D^*,\mf u_A^*)$ are at a saddle-point equilibrium, and the value of the game is $Q^*(\mf z_0) = \Qest(\mf z_0)$.
\end{corollary}
If the intruders stick to $\mf u_A^*$, then the defender team cannot reduce the score by changing their strategy.
Similarly, if the defenders keep $\mf u_D^*$, then the intruders cannot increase the score by changing their strategy.
% This result indicates the optimality of the proposed strategy in the sense that any deviation does not improve the score as long as the opponent sticks to the equilibrium strategy.


==> defense_policy_old.tex <==
\section{DEFENSE POLICY  \label{sec:defense_policy}}

\daigo{This section is going to change significantly including some of the results (algorithms and proofs), however the conclusion on the saddle point equilibrium stays the same.}

\noindent This section proposes the defender team strategy that outperforms the existing ones.
We first present the algorithm and then prove the condition when all intruders are captured.
Finally, we show that the score is bounded from above by $\Qest$ under certain condition, indicating that $\Qest$ is the outcome of the game.

\subsection{The LGR-defense Algorithm}
\noindent
Our algorithm visits each intruder once and decides a defender or a defender pair to be assigned to it.
To narrow down the selection of the defender for a given intruder, we identify a unique I-LGR for each intruder as follows.

We first extend the concept of LGS defined for LGRs in Lemma~\ref{lem:lgs} to I-LGRs.
The \emph{independent local game score} (I-LGS) is defined as
\bql
\lgsi_k \triangleq \hat{n}_A^k - n_D^k =  q_k + \Delta n_A^k,
\eql
where $\Delta n_A^k$ is the number of intruders in the paired defense region $\dwinrp^k$.

The local game score of $q_k=0$ was a critical number in Sec.~\ref{sec:QLG} since it meant that any additional intruder in the LGR will immediately lead to a positive intruder score (Lemma~\ref{lem:lgs}). 
We say that $k$th LGR (resp.~I-LGR) is \emph{occupied} if $q_k\geq 0$ (resp.~$\lgsi_k\geq 0$): every defender in the region needs to capture one intruder to avoid intrusion.
Consider the set of all occupied I-LGRs that contains $A_i$:
\bql
\mf k^{(i)} = \{ k \;|\; \lgsi_k \geq 0, \text{\;and\;} \mf x_{A_i} \in \awinrci^k\}.
\eql
When $\mf k^{(i)} \neq \emptyset$, we define a mapping $\pi: \ateam \rightarrow \{1,...,N_D^2\}$ from an intruder to an I-LGR as follows:
\bnl
&\pi(i)  = \argmin \limits_{k\in \mf k^{(i)}} n_D^k
\enl
i.e., $\pi(i)$ gives the index of the smallest, occupied I-LGR that contains $A_i$.
In the degenerate case when $\mf k^{(i)}=\emptyset$, such I-LGR is not well defined; we use $\pi(i)=\emptyset$.

The I-LGS has another critical number: $\lgsi_k=1$.
Unlike $q_k=1$, this configuration does not immediately lead to intruder score.
To see this, suppose $q_k \leq 0$ and $\lgsi_k = 1$, then one intruder in $\dwinrp^k$ can be captured by the pincer maneuver of the boundary defenders, and the rest may be captured by the defender subteam $\subteam_D^k$.


The LGR defense strategy is presented in Algorithm~\ref{alg:LGRdefense}. 
% ALGORITHM:
\begin{algorithm}[t]
\caption{LGR Defense \label{alg:LGRdefense}}
\begin{small}
\begin{algorithmic}[1]
\State Remove $\aignore$ using Algorithm~2
\State Find smallest I-LGR for each intruder: i.e., $\pi (i)$
\State Sort them in ascending order with respect to $n_D$

\For {$k$ in $ \{\pi(i)\}_{i=1}^{N_A}$ }
        \If {$\lgsi_k=1$}
	        \State Select one intruder in $\dwinrp^k$ and assign to $D_B^k$
        \EndIf
        \State Find free intruders and defenders in $\awinrci^k$    
	\State Matching of those agents
\EndFor
\State Matching of remaining agents
\State {\bf Return}: assignments (i.e., direction of motion)
\end{algorithmic}
\end{small}
\end{algorithm}
In the first line, the intruders that are guaranteed to score are ignored so that the defenders can focus on the rest (to be discussed in Sec.~\ref{sec:saddle_point}).
Both individual defense (1v1) and cooperative defense (2v1) are considered.

\todo{Example}
When a defender has an individually assigned intruder, then that is the only assignment that the defender has.
However, if a defender is assigned a 2v1 defense, it could potentially have multiple 2v1 games assigned to it.
This is one of the main differences from the previous defense strategies (MM or MIS approach), and will be explained in detail in the next subsection.
We will show that such overlapping assignments all require the same direction of motion from the defender, and will eventually dissolve into multiple 1v1 games.


Each intruder has either one of the following: (i) one defender assigned, (ii) a pair of defenders assigned, or (iii) no defender assigned.
Another major difference from the existing defense policies is that, with our algorithm, even those intruders without explicit assignment at the current time can be shown to be captured when certain conditions are met.
In fact, we will show in the next section that all intruders will be captured if $\Qest=0$ and $\lgsi_k\leq 1,\; \forall\, k$.


% Perfect defense
\subsection{Conditions for Perfect Defense}
\noindent
This section discusses the condition in which LGR defense (Algorithm~\ref{alg:LGRdefense}) leads to the capture of all intruders.
If a defender or a defender pair is assigned to a unique intruder, it is clear that the intruder is guaranteed to be captured.
There are two additional types of engagements in the LGR-defense: the \emph{unassigned defense} and the \emph{sequential paired defense}.


% Figure: unassigned defense
\begin{figure}[h]
\centering
\includegraphics[width=.49\textwidth]
{figures/unassigned_defense}
\caption{Unassigned defense structure.
(a) Initial configuration where $A_2$ is in the unassigned-defense zone.
(b) The structure is resolved into two 1v1 assignments.
}
\label{fig:unassigned_defense}
\end{figure}
%
% \begin{definition}
The \emph{unassigned defense} structure is a two vs.~two engagement within an I-LGR where one intruder is in $\dwinrp(i,j)$, and the other is in $\dwinr(i)\cap\dwinr(j)$ (see Fig~\ref{fig:unassigned_defense}a).
% \end{definition}
Algorithm~\ref{alg:LGRdefense} assigns the pair ($\di,\dj$) to $A_1$, but no defender to $A_2$ because there is no free defender for the 1v1 assignment nor it is in $\dwinrp(i,j)$ for the 2v1 assignment.
Nevertheless, the intruder in this position will eventually get a unique 1v1 assignment.

\begin{lemma}\label{lem:unassigned_defense1}
The \emph{unassigned defense} structure will turn into two 1v1 assignments in finite time.
\end{lemma}
\begin{proof}
From the 2v1 assignment against $A_1$, $\di$ moves ccw and $\dj$ moves cw.
Under this movement, $A_2$ remains in $\dwinr(i)\cap\dwinr(j)$ because it cannot penetrate $\di$'s left barrier nor $\dj$'s right barrier (Prop.~\ref{prop:1v1barrier}).
Before they meet at the midpoint, $A_1$ will move into either $\dwinr(i)$ or $\dwinr(j)$ (Prop.~\ref{prop:pincer}).
Suppose w.l.o.g. $\mf x_{A_1}\in \dwinr(i)$, then $A_2$ will get 1v1 assignment to $\dj$. 
\end{proof}

\begin{lemma}\label{lem:unassigned_defense2}
If $\Qest= 0$ and $\lgsi\leq1$, then every unassigned intruder is in a unique \emph{unassigned defense} structure: i.e., they will all be captured.
\end{lemma}
\begin{proof}
\todo{complete}
Let $X$ be the set of unassigned intruders, and $Y$ be the set of outer-most defender pairs performing 2v1 games.
The neighbors $\mc{N}(x)$ of $x\in X$ are pairs in $Y$ that contains $x$ in the unassigned defense zone.
We use Hall's marriage theorem, which states that there is an $X$-saturating matching iff every subset $W$ of $X$ has sufficiently many adjacent vertices in $Y$.
Suppose there exists $W\subset X$ such that $|W|>|\mc{N}(W)|$.
Then find the first pair in $Y\setminus\mc{N}(W)$ on the ccw and cw side of $W$.
Consider the I-LGR defined by the left B.D.\ of ccw pair and right B.D.\ of cw pair.
It can be seen that the I-LGS of that region is $\lgsi = |W|-\mc{N}(W)\geq 1$.
This violates the assumption that pairs in $Y$ are all outer-most pairs.
By contradiction we showed that $|W|\leq|\mc{N}(W)|$.
By Hall's theorem, there is a unique pair for every unassigned intruder.
\end{proof}


The \emph{sequential paired defense} occurs when a defender has multiple 2v1 assignments.
(Note that Algorithm~\ref{alg:LGRdefense} prohibits a single defender to have both 1v1 and 2v1 assignments, but does allow a defender to have multiple 2v1 assignments.)
% Figure: sequential 2v1
\begin{figure}[h]
\centering
\includegraphics[width=.49\textwidth]
{figures/sequential_2v1}
\caption{
Sequential 2v1 structure.
(a) The defender $D_j$ has two 2v1 assignments, and cw motion is required for both.
(b) The structure is resolved into two 1v1 assignments.
}
\label{fig:sequential_2v1}
\end{figure}
%
\begin{lemma}\label{lem:sequential_2v1}
Suppose Algorithm~\ref{alg:LGRdefense} assigned multiple 2v1 games to $\di$.
If $\Qest=0$ and $\lgsi_k\leq1,\,\forall\,k$, then all those assignments require the same direction of motion by $\di$.
\end{lemma}
\begin{proof}
If $D_i$ serves as the left (or right) boundary defender for all of the 2v1 assignments, then the required motion is the same for all.
We show by contradiction that $D_i$ does not serve as the left and right boundary defender simultaneously.

Suppose $D_L^l = \di$ and $D_R^r=\di$: $l$ and $r$ denote the indices of the LGRs that $\di$ serves as the left and right boundary defender, with $q_l=q_r=0$ and $\lgsi_l=\lgsi_r=1$.
There are two cases: (i) $\awinrc^{l}\cap\awinrc^{r}=\emptyset$, and (ii) $\awinrc^{l}\cap\awinrc^{r}\neq\emptyset$.

In the first case let $m$ denote the smallest LGR that contains both $l$ and $r$.
Since $n_A^m\geq (n_A^l+1)+(n_A^r+1)$, we have
$q_m = n_A^m-n_D^m
\geq (n_D^l+1)+(n_D^r+1)-(n_D^l+n_D^r+1)
=1$,
which contradicts with $\Qest \leq 0$.
The second case can be proved similarly, where the condition $\lgsi_k\leq 1$ is used to bound the number of intruders in the intersection.
\end{proof}

Fig.~\ref{fig:sequential_2v1}a shows an example of sequential paired defense configuration.
Multiple defenders are interrelated through the pairing for cooperative defense.
Recalling the 2v1 analysis, the intruder in $\dwinrp$ will eventually move into the defender winning region of either of the two boundary defenders.
Every time such transition occurs, the number of interrelated 2v1 game decreases, and we have additional 1v1 and/or implicit assignment configuration.
%Consider a structure with $m$ interrelated cooperative defense.
%We know that there are $m$ intruders and $m+1$ defenders.
%After one transition, we will have either of the following:
%\begin{itemize}
%\item One 1v1  and $m-1$ interrelated 2v1 
%\item One \emph{implicit} and $m-2$ interrelated 2v1 
%\item Two 1v1  and $m-2$ interrelated 2v1 
%\item One 1v1, one \emph{implicit}, $m-3$ interrelated 2v1, and one free defender
%\end{itemize}
%In any of the above cases, the number of interrelated 2v1 game decreases.
%Eventually they all turn into 1v1 or the implicit assignment.
% Again, such favorable transitions are possible because all pairs are moving optimally against all of the assigned intruders.

\begin{theorem}\label{thm:perfect_defence}
If the initial configuration is such that $\Qest=0$ and $\lgsi_k\leq 1, \forall\,k$, then the LGR-defense (Algorithm~\ref{alg:LGRdefense}) guarantees perfect defense.
\end{theorem}
\begin{proof}
The intruders have either (i) a unique 1v1 assignment, (ii) 2v1 assignment, or (iii) no assignment.
By construction, every 1v1 assignment guarantees capture.
Lemmas~\ref{lem:unassigned_defense1} and \ref{lem:unassigned_defense2} prove that intruders with no assignment will all be captured. 
Lemma~\ref{lem:sequential_2v1} and the discussion that follows prove that all 2v1 assignments will lead to capture.
\end{proof}

% Saddle point equilibrium
\subsection{Saddle-point equilibrium}
\label{sec:saddle_point}
\noindent This section addresses the case when the intruder team can guarantee non-zero score: $\Qest>0$.
The idea behind the first line in Algorithm~\ref{alg:LGRdefense} is to ignore the intruders that cannot be captured, and make sure all other intruders are captured.
\begin{lemma}\label{lem:removal}
Suppose $\Qest=n>0$, then there exists a set of $n$ intruders whose removal will generate a new game with $\Qest=0$.
\end{lemma}
\begin{proof}
We show by contradiction that there exists an intruder whose removal decreases $\Qest$ by one.
Suppose there is no such intruder.
Then there exists at least two sets $\djset_1^*$ and $\djset_2^*$ that gives the optimal score $Q(\djset_1^*) = Q(\djset_2^*) = \Qest$, with the constraint $\subteam_A^k\cap\subteam_A^l=\emptyset$ for $k\in\djset_1^*$ and $l\in\djset_2^*$, i.e., no common intruders.
The two sets do not share any intruder because if they did, then the removal of the common intruder will reduce both $Q(\djset_1^*)$ and $Q(\djset_2^*)$.

Now, take $k\in\djset_1^*$ with $q_k>0$ and consider merging it to $\djset_2^*$.
If $\awinrc^k\cap\awinrc^l=\emptyset$ for $\forall\, l\in\djset_2^*$, then $\djset_3 = \{k,\djset_2^*\}$ is a valid disjoint set and it has $Q(\djset_3)>Q(\djset_2^*)$, which contradicts with the optimality of $\djset_2^*$.
If $k$ intersects with $l\in\djset_2^*$, then let $m$ be the smallest LGR that contains both $k$ and $l$.
Since the regions intersect, we have $n_D^m<n_D^k+n_D^l$.
However, since they share no intruders, we have $n_A^m\geq n_A^k+n_A^l$.
Therefore, $q_m= n_A^m-n_D^m > n_A^k+n_A^l- n_D^k-n_D^l = q_k+q_l$, which again contradicts with the optimality of $\djset_2^*$.
The case when $k$ intersects with multiple LGRs in $\djset_2^*$ can be treated similarly.

Repeating the same process $n$ times, the score $\Qest$ reduces to zero after removing $n$ intruders.
Also, observe that the order of the removal does not affect the result.
% Consider the optimally selected disjoint set $\mf G^*$.
% For an LGR with $q_k\geq 1$ in $\mf G^*$, we show by contradiction that there exists an intruder whose removal makes $q_i\leq q_k-1$ for all $i$ such that $\awinrc^i\subseteq\awinrc^k$; i.e., $\Qest$ is reduced by one.
% Suppose there is no such intruder.  
% Then we should have at least two LGRs $\awinrc^i$ and $\awinrc^j$ contained in $\awinrc^k$ that satisfy the following conditions: (i) $q_i=q_j=q_k$, and  (ii) $\subteam_A^i\cap\subteam_A^j=\emptyset$.
% If the two LGRs are disjoint, then $q_i+q_j = 2q_k > q_k$ contradicts with the assumption that $k\in G^*$ (we would have $i,j\in \mf G^*$ instead).  
% If the two LGRs intersect, let $\awinrc^m\subseteq \awinrc^k$ be the smallest LGR that contains both $\awinrc^i$ and $\awinrc^j$.
% One can show that this leads to a contradiction $q_m>q_k$.
% After removing one intruder, we can choose the next LGR in $\mf G^*$ with $q>0$ and repeat the process until $q_k\leq0,\,\forall\,k$.  Since each removed intruder contributes to the reduction in $\Qest$, at most $\Qest$ intruders need to be removed.
\end{proof}

Let $\aignore$ be a set of intruders with cardinality $|\aignore|=\Qest$, such that removal of those intruders generate a new game with $\Qest=0$.
Following the proof of Lemma~\ref{lem:removal}, one can find $\aignore$ by visiting every intruder and asking whether it reduces $\Qest$ or not (Algorithm~\ref{alg:removal}).
Since each intruder is visited at most once, Algorithm~\ref{alg:removal} terminates within less than $N_A$ iteration.
% Every time the answer is yes, we remove that intruder from the game, and continue until $\Qest=0$.
% Assuming that the set $\djset^*$ is already known, the complexity is linear in $N_A$ since each intruder is visited only once.
% ALGORITHM:
\begin{algorithm}[t]
\caption{Removal of uncapturable intruders \label{alg:removal}}
\begin{small}
\begin{algorithmic}[1]
\State Initialize: $\aignore=\emptyset$, and $i=1$ 
\While {$\Qest>0$}
    \State $Q_{new}\gets$ compute $\Qest$ without $\{A_i,\aignore \}$
    \If {$Q_{new} < \Qest$}
        \State append $A_i$ to $\aignore$
        \State $\Qest\gets Q_{new}$
    \EndIf
    \State $i\gets i+1$
\EndWhile
\State {\bf Return}: $\aignore$
\end{algorithmic}
\end{small}
\end{algorithm}


\begin{theorem}
If $\hat{q}_k\leq 1\,\forall\,k$ after removing $\Qest$  intruders found by Algorithm~\ref{alg:removal}, then the LGR-defense policy $\mf u_D^*$ guarantees
\bql
Q(\mf u_D^*,\mf u_A)\leq  \Qest, \; \forall \, \mf u_A\in U_A,
\label{eq:uDguarantee}
\eql
where $U_A$ is the set of all permissible intruder strategies.
\end{theorem}
\begin{proof}
The result immediately follows from Theorem~\ref{thm:perfect_defence} and Lemma~\ref{lem:removal}.
\end{proof}

Finally, the combination of the strategy $\mf u_A^*$ from Theorem~\ref{thm:Qlow} and $\mf u_D^*$ from Theorem~\ref{thm:perfect_defence} gives us the following result:
\bql
Q(\mf u_D^*,\mf u_A)\leq  Q(\mf u_D^*,\mf u_A^*) \leq Q(\mf u_D,\mf u_A^*),
\eql
i.e., the strategies $(\mf u_D^*,\mf u_A^*)$ are at a saddle-point equilibrium, and the value of the game is $Q(\mf u_D^*,\mf u_A^*) = \Qest$.
This result indicates the optimality of the proposed strategy in the sense that any deviation from the optimal strategy does not improve the score as long as the opponent sticks to the equilibrium strategy.

